Testing Lepton Flavor Universality and CKM Unitarity with Rare Pion Decays in the PIONEER experiment

The physics motivation and the conceptual design of the PIONEER experiment, a next-generation rare pion decay experiment testing lepton flavor universality and CKM unitarity, are described. Phase I of the PIONEER experiment, which was proposed and approved at Paul Scherrer Institut, aims at measuring the charged-pion branching ratio to electrons vs.\ muons, $R_{e/\mu}$, 15 times more precisely than the current experimental result, reaching the precision of the Standard Model (SM) prediction at 1 part in $10^4$. Considering several inconsistencies between the SM predictions and data pointing towards the potential violation of lepton flavor universality, the PIONEER experiment will probe non-SM explanations of these anomalies through sensitivity to quantum effects of new particles up to the PeV mass scale. The later phases of the PIONEER experiment aim at improving the experimental precision of the branching ratio of pion beta decay (BRPB), $\pi^+\to \pi^0 e^+ \nu (\gamma)$, currently at $1.036(6)\times10^{-8}$, by a factor of three (Phase II) and an order of magnitude (Phase III). Such precise measurements of BRPB will allow for tests of CKM unitarity in light of the Cabibbo Angle Anomaly and the theoretically cleanest extraction of $|V_{ud}|$ at the 0.02\% level, comparable to the deduction from superallowed beta decays.

==> Appendices/Authors.tex <==

{\bf PIONEER Collaboration}


\author[23]{W. Altmannshofer}
\author[12]{H. Binney}
\author[28]{E. Blucher}
\author[2,3]{D. Bryman}
\author[6] {L. Caminada}
\author[6] {S. Corrodi}
\author[4]{S. Chen}
\author[5]{V. Cirigliano}
%\author[6,7,8]{A. Crivellin}
\author[9]{ S. Cuen-Rochin}
\author[10]{A. Czarnecki}
\author[19] {A. DiCanto}
\author[11]{L. Doria}
\author[29] {A. Fienbert}
\author[24] {A. Gaponenko}
\author[12]{A. Garcia}
\author[13]{L. Gibbons}
\author[14]{C. Glaser}
\author[11]{M. Gorchtein}
\author[15]{T. Gorringe}
\author[23]{S. Gori}
\author[23]{A. Grillo}
\author[12]{D. Hertzog}
\author[12]{ Z. Hodge}
\author[16]{ M. Hoferichter}
\author[18]{S.  Ito}
\author[17]{T. Iwamoto}
\author[19] {D. Jaffe}
\author[12]{ P. Kammel}
\author[12]{J. Kaspar }
\author[19] {S. Kettel}
\author[24] {B. Kiburg}
\author[6] {A. Knecht}
\author[26]{T. Koffas} 
\author[13]{ K. Labe}
\author[12]{J. LaBounty}
\author[6] {U. Langenegger}
\author[8]{ C. Malbrunot}
\author[19]{ W. Marciano}
\author[23] {S. M. Mazza}
\author[20]{ S. Mihara}
\author[3]{ R. Mischke}
\author[17]{T. Mori}
\author[19] {J. Mott}
\author[12] {E. Muldoon}
\author[3]{T. Numao }
\author[17]{ W. Ootani}
\author[1]{ C. Ortega Hernandez}
\author[3] {K. Pachel}
\author[14]{ D. Po\v{c}ani\'c}
\author[24]{C. Polly}
%\author[3] {F. Retiere}
\author[11] {D. Ries}
\author[12] {R. Roehnelt}
\author[21]{ D. Salvat}
\author[23] { B. Schumm}
\author[6] {P. Schwendimann}
\author[23] { A. Seiden}
\author[25] {A. Soter}
%\author[3] { A. Sher}
\author[27] {R. Shrock}
\author[22]{T. Sullivan}
\author[12] {D. Sweigart}
\author[19] {V. Tischenko}
\author[19] { A. Tricoli}
\author[3]{B. Velghe}
\author[17] {T. Wataru}
\author[12] {C. Welch}
\author[3] {V. Wong}
\author[19] {E. Worcester}




\affiliation[1]{Universidad Nacional Autonoma de Mexico}
\affiliation[2]{University of British Columbia}
\affiliation[3]{TRIUMF}
\affiliation[4]{Tsinghua University}
\affiliation[5]{Los Alamos National Laboratory}
\affiliation[6]{Paul Scherrer Institute}
\affiliation[7]{University of Zurich}
\affiliation[8]{CERN}
\affiliation[9]{Universidad Autonoma de Sinaloa}
\affiliation[10]{University of Alberta}
\affiliation[11]{Johannes Gutenberg University of Mainz}
\affiliation[12]{University of Washington}
\affiliation[13]{Cornell University}
\affiliation[14]{University of Virginia}
\affiliation[15]{University of Kentucky}
\affiliation[16]{University of Bern}
\affiliation[17]{University of Tokyo}
\affiliation[18]{Okayama University}
\affiliation[19]{Brookhaven National Laboratory}
\affiliation[20]{KEK}
\affiliation[21]{Indiana University}
\affiliation[22]{University of Victoria}
\affiliation[23]{University of California Santa Cruz}
\affiliation[24]{Fermilab }
\affiliation[25]{ETH Zurich}
\affiliation[26]{Carleton University}
\affiliation[27]{Stoney Brook University}
\affiliation[28]{University of Chicago}
\affiliation[29]{Pennsylvania State University}


==> Appendices/LYSO-alt.tex <==
\section{Alternative LYSO Calorimeter Considerations}
A naturally segmented array of tapered LYSO crystals provides an attractive alternative to our proposed LXe-based calorimeter.  We are exploring a geometry that matches that of the PEN pure CsI detector. The PEN crystals were limited to 12$X_0$  depth, which is insufficient for an ideal $\pi \rightarrow e \nu$ measurement.  However, the segmentation and fast response allows for various trigger patterns and it is well-designed for the pion beta decay phase in the PiBeta configuration. This detector has an inner radius of 26\,cm, and an outer radius of 48\,cm.  CsI has a radiation length of 1.86\,cm. With the compact ATAR geometry we are proposing, a sufficient volume exists to insert an inner array of crystals between the ATAR and the existing PEN CsI array, see Fig.~\ref{fig:detector_PEN} and Fig.~\ref{fig:LYSO-figs}a.   On paper, LYSO crystals appear to be the ideal choice for such an array.  LYSO is a Cerium doped Lutetium based scintillator whose light output is comparable to doped NaI(Tl).  It has high density ($X_0$= 1.14\,cm, $R_{M}$=2.07 cm) and a light yield comparable to the highly luminous NaI(Tl), but with much faster light signals.  Its 420\,nm typical scintillation light has a 40\,ns single exponential decay time and the spectrum is well matched to conventional SiPM photosensors.  LYSO is both radiation hard and non-hygroscopic. To date, the main application for LYSO crystals has been in PET medical scanners, where small crystals are needed with high light output to resolve the 511\,keV gammas from positron annihilation.  The attractive properties of these crystals suggest that larger arrays could be made for use in particle physics applications and, indeed, several groups have explored this possibility with small arrays and somewhat limited success.

Experts in the field, such as Ren-Yuan Zhu from Caltech, have advised our collaboration on the pros and cons and experiences of other groups, see for example \cite{Zhu:2021sij}.  The growth of relatively long LYSO crystals is a fairly new and expensive R\&D effort, not easily justified without a demanding end-use application.  The Mu2e Collaboration built a $5 \times 5$ array of $3 \times 3 \times 20\,$cm$^3$ crystals and subjected the array to test beams at Frascati and Mainz~\cite{Atanov:2016blu}.  At 100\,MeV, the resolution was in the range of 3--4\%,  dominated by a 2.5\% constant term indicative of non-uniformity in light transmission and possibly crystal to crystal calibrations and surface preparation.  That performance met the specifications for Mu2e, but they did not push it further, choosing eventually to use undoped CsI based on an overall cost analysis.
\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{Figures/LYSO-figs.pdf}
\caption{Possible use of an inner array of tapered LYSO crystals within the open volume of the existing PEN CsI calorimeter.  a) Opened view showing in blue the array of LYSO crystals that matches one-to-one to the existing geometry of the PEN crystals shaded in gray.  b) An example array ideal for testing the concept.  c) An individual pentagonal crystal, 16$X_0$ in depth.  Each such crystal would be read out by a thin array of SiPMs.
}
\label{fig:LYSO-figs}
\end{figure}

Dr. Zhu has investigated crystals from various companies and published properties that will guide us going forward.  An example of a study of a 25$X_0$ crystal's longitudinal transmission and how to improve it is found in \cite{Mao:2012dr}.  It is imperative to improve on the uniformity of light production and transmission along the length of the crystal.  Experience has shown -- as it has for CsI -- that custom surface preparation on tapered crystals is also important and can be realized with careful lab bench work.  We aim to investigate the possibilities of using LYSO for PIONEER, but would not now claim this to be defensible until proper bench tests and manufacturer quotes are in hand.  Figures\,\ref{fig:LYSO-figs}b and c indicated prototype geometries that are designed to fit inside the PEN calorimeter.  We will issue requests to a variety of companies for quotes to see if these crystal shapes can be made to meet our specifications.
If tests are successful --- principally achieving the needed energy resolution below 3\% -- then a careful side-by-side comparison of costs and performance against our leading calorimeter candidate based on LXe can be made.







==> Appendices/inTargetDifSuppression.tex <==
\section{In-target Decay-in-flight $\pi \rightarrow \mu \nu$ Suppression with BDT}
\label{sec:DIFsuppression_BDT_appendix}

\begin{itemize}
    \item plots of input features (pienu vs DIF)
    \item BDT score distribution
    \item ROC curve
    \item suppression factor with the consideration of energy smearing
\end{itemize}

==> Appendices/pibetaReview.tex <==
\section{PiBeta}

{\bf Pion beta decay measurements}

The branching ratio for pion beta decay was most accurately measured by the PiBeta experiment\footnote{The PiBeta and PEN experiments shared much of the same apparatus.} at PSI \cite{Pocanic1,Frlez:2003vg,Pocanic:2003pf,Frlez:2003pe,Bychkov:2008ws} to be
$\frac{\Gamma(\pi^+ \to  \pi^0 e^+ \nu)}{\Gamma\textrm{(Total)}}= [1.036 \pm 0.004 \textrm{(stat)} \pm 0.004\textrm{(syst)} \pm 0.003(\pi\to e\nu)] \times 10^{-8}$, where the first uncertainty is statistical, the second systematic, and the third is the $\pi\to e\nu$ branching ratio uncertainty.
Pion beta decay potentially provides the theoretically cleanest determination of the magnitude of the CKM matrix element \vud. With current input one obtains $\vud = 0.9739(28)_{\textrm{exp}}(1)_{\textrm{th}}$, where the experimental uncertainty comes almost entirely from the  $\pi^+ \rightarrow \pi^0 e^+ \nu (\gamma)$ branching ratio (BRPB).
%(the pion lifetime contributes ${\delta}V_{ud} = 0.0001$).
The theory uncertainty has been reduced from $({\delta}V_{ud})_{\textrm{th}} = 0.0005$ \cite{Sirlin:1977sv, Cirigliano:2002ng, Passera:2011ae} to $({\delta}V_{ud})_{\textrm{th}} = 0.0001$ via a lattice QCD calculation of the radiative corrections \cite{Feng:2020zdc}. The current precision of \unit[0.3]{\%} on \vud makes $\pi^+ \rightarrow \pi^0 e^+ \nu (\gamma)$ not presently relevant for the CKM unitarity tests because super-allowed nuclear beta decays provide a nominal precision of %0.015\%. 
\unit[0.03]{\%}. 
In order to make $\pi^+ \rightarrow \pi^0 e^+ \nu (\gamma)$ important for CKM unitarity tests, two precision experimental stages can be identified:
%\begin{enumerate}  
(1) As advocated in Ref.~\cite{Czarnecki:2019mwq}, a three-fold improvement in BRPB precision compared to Ref.~\cite{Pocanic:2003pf} would allow for a 0.2\% determination of $\left|V_{us}/V_{ud}\right|$ improving on measurement of the following ratio being currently 
 %   \begin{equation}
      $  R_V = \frac{\Gamma\left(\textrm{K} \rightarrow \pi l \nu (\gamma) \right)}{\Gamma\left(\pi^+ \rightarrow \pi^0 e^+ \nu (\gamma)\right)}=1.3367(25)$ ,
 %   \end{equation}
    independent of the Fermi constant, short-distance, and structure-dependent radiative corrections. This
    would match the precision of the current extraction of $\left|V_{us} / V_{ud}\right|$ from the axial channels~\cite{Marciano:2004uf} 
  % \begin{equation}
        $R_A = \frac{\Gamma\left(\textrm{K} \rightarrow \mu \nu (\gamma) \right)}{\Gamma\left(\pi \rightarrow \mu \nu (\gamma)\right)}=1.9884(115)(42)$,
 %   \end{equation}
  providing a new competitive constraint on the \vus--\vud\ plane and probing new physics that might affect vector and axial-vector channels in different ways.
    The theoretical case for this approach was recently strengthened by improved analysis of radiative corrections in $K \to \pi e \nu $ decays \cite{Seng:2021nar}.  
(2)  In the second phase, an order of magnitude improvement  in the
BRPB precision will be sought. This would provide the theoretically cleanest extraction of \vud at the \unit[0.02]{\%} level. 

==> DAQ/daq.tex <==
\subsubsection{Data acquisition system}

The PIONEER data acquisition system must handle the read out, event assembly and data storage for the active target, positron tracker, electromagnetic calorimeter and other detector sub-systems of the experimental setup. It must provide a deadtime-free, distortion-free record of the datasets identified by the various physics and calibration triggers. It must facilitate the monitoring needed to guarantee the overall integrity of data taking and provide the metadata needed to document the experimental configuration during data taking. Finally, it must enable the configuration of the readout electronics and the associated trigger, clock and control system.

The acquisition will be implemented as a modular, distributed system on a parallel, layered processor array consisting of networked, multi-core, commodity PC's running a scientific Linux operating system. The overall layout is depicted schematically  in Fig.\ \ref{f:daqlayout}.  It will comprise a frontend processor layer responsible for readout and processing of event fragments from the FPGA-based fast electronics instrumenting the various detector sub-systems, a backend layer responsible for event building and data storage,  a slow control layer responsible for configuration and readback, and a data quality layer responsible for monitoring of data integrity.

To maximize the bandwidth the frontends will utilize memory-mapped, Gen3 PCI Express communication with the Apollo readout boards and the downstream DAQ layers will utilize memory-mapped, Gen3 PCI Express host / target adaptors for data transfer and sharing system resources (disks, GPUs, {\it etc}). PCI-Express 3.0 delivers an effective data transfer rate of nearly 1 GB/s per serial lane. Commercial host-to-target optical interfaces are now available for the Apollo FPGA to frontend computer communication ({\it e.g.}, www.dolphinics.com/products/PXH842.html). Commercial peer-to-peer communication is also now available for direct PCI-Express data transfer between devices ({\it e.g.}, www.dolphinics.com/products/PXH810.html).   The setup will offer the capability of direct transfer of  data to / from FPGA and CPU / GPU memory for rapid realtime processing. 

\begin{figure}[t!]
\includegraphics[width=0.99\textwidth]{Figures/DAQschematic.png}
\caption{Schematic of the data acquisition system showing the frontend layer for data readout and experiment configuration, the backend layer for event assembly and data storage, and the analysis layer for data quality monitoring. The number of frontends and the topology of the FPGA-to-frontend and frontend-to-backend networks will be based on the calorimeter, ATAR and FPGA technology choices.}
\label{f:daqlayout}
\end{figure}

The DAQ software will be based on the MIDAS data acquisition package \cite{midas}, CUDA GPU toolkit \cite{cuda}, ROOT data analysis package \cite{root}, and Linux PCI Express system and utility libraries. The MIDAS software consists of library functions for data flow between different processes on local / remote devices as well as infrastructure for data logging, experimental configuration and local /remote run control. It also incorporates an integrated alarm system and slow control system. The devices drivers for the configuration and the readout of the Apollo board FPGAs will be based on the PCI Express communication protocols / libraries.

As discussed in Sec.~\ref{Trigger} and Table~\ref{tab:triggers}, we anticipate the various physics triggers to include a prescaled beam trigger \tpi, a beam particle - high energy \calo\ trigger \tcaloh, a prescaled beam particle - low threshold \calo\ trigger \tprompt, and a beam particle - outgoing positron trigger \ttrack ~(as identified by either the ATAR or the tracker). The cumulative trigger rate in Table~\ref{tab:triggers} is estimated at approximately 8.8\,kHz. 

The ATAR data will comprise above-threshold islands of contiguously digitized ADC samples from the fired detector strips of the active stopping target. Based on a 1 GSPS sampling rate, 4 Bytes per sample, and 66 above-threshold strips per trigger, we anticipate an \atar\ data rate of about 70~MB/s for the aforementioned trigger types.

The CALO data  will comprise islands of contiguously digitized ADC samples from the SiPM / PMT readout of the calorimeter. Based on a 1 GSPS sampling rate, 2 Bytes per sample, 200 samples per island and 1000 islands / channels per trigger, we anticipate a \calo\ data rate of about 3.5 GB/s for the aforementioned trigger types.

Other detector systems will include the various beam detectors upstream of the ATAR and the positron tracking detector surrounding the ATAR. The data rates from beam detectors and tracking detector are expected to be a small fraction of the ATAR / CALO data rate.

Separate frontend processors running  MIDAS frontends will readout the ATAR, calorimeter, tracker and beam sub-systems via the  PCI-express bus using commericial transparent host / target PCI Express adapters to the Virtex FPGAs on the Apollo readout boards. The memory-mapped readout from the Virtex FPGAs chip will permit both high data transfer rates and direct data transition to system CPU and GPU memories. We plan to utilize IPBus over PCI Express for the configuration of the readout electronics and the trigger, clock and control system.

The data acquisition system will process in real-time the data from a roughly 3.5 GB/sec raw data rate to a roughly $\sim$300 MB/sec processed data rate for data storage on PSI's Petabyte archive. One option for the data processing is the lossless compression of the slow decay-time calorimeter signals via a combination of delta encoding and Golomb coding. The delta encoding will exploit the correlations between sequential ADC samples to shrink the word usage distribution while Golomb coding is suited to situations in which the occurrences of small values are significantly more likely than the occurrences of large values. Other possibilities are zero suppression of \calo\ islands and realtime fitting of \calo\ pulses. These algorithms are well suited to parallel processing using GPUs.

We are initiating an R\&D effort to demonstrate both the technology for the FPGA-to-CPU / GPU communication via optical PCI-express links and the performance of the data compression schemes. The R\&D setup will allow for code development, testing and debugging as well as the evaulation of the rate capabilities and the compression capabilities of the system. We plan to use commercial PCI-Express FPGA development boards as data simulators for the detector sub-systems in order to prototype and benchmark the DAQ.

The PIONEER DAQ group has developed and operated similar architectures of distributed data acquisition systems for the MuLan, MuCap and MuSun experiments at the Paul Scherrer Institute and the g-2 experiment at Fermi National Accelerator Lab.


%\subsubsection{Data Policy}

%The PIONEER collaboration will comply with the \emph{data policy for PSI research data} \cite{PSIdataPolicy} and will publish the experiment's data under PSI's custody after a suitable embargo period. We are also committed to publish our software under an open source license at a suitable time.



==> PioneerExperiment/ATAR/ATAR.tex <==
\label{sec:ATAR}

%The ATAR, having a few mm of active thickness, would be sitting at the most probable pion interaction point and the calorimeter would be a sphere of a 1~m radius around it.
%A schematic of PIONEER external enclosure can be seen in \cref{fig:PIONEER}, left. The ATAR region is highlighted in red in the shown schematic. The following sections will be focused on the ATAR detector development.

%The ATAR would provide a high precision 4D tracking that would allow to separate the energy deposits of the pion decay products in both position and time. Furthermore it will allow to suppress other significant systematic uncertainties (pulse pile-up, decay in flight of slow pions) to $<$~0.01\%.
%The combination of the high precision calorimeter and the ATAR will allow the overall uncertainty in the measurements of $R_{e/\mu}$ and Pib to be reduced to O(0.01\%) and O(0.05\%) respectively.
%For the $R_{e/\mu}$ phase $3\times10^5$ $\pi^+$ per second (around $10^{12}$~total $\pi^+$ per year) are expected, for the Pib phase $1.5\times10^7$ $\pi^+$ per second (around $10^{14}$~total $\pi^+$ per year) are expected.

%Pions come to rest in a highly segmented active target (ATAR) and decay to muons or positrons. The present concept for the ATAR includes 48 layers of orthogonal LGAD strips, $\unit[120]{\mu m}$ thick with pitch of $\unit[200]{\mu m}$. Prototypes made at Brookhaven National Laboratory are being investigated at U.~C.~Santa Cruz and eventually will be tested at TRIUMF. The segmentation of the target is crucial in defining the fiducial region for  pion stops, handling the high rate for $\pi^+ \to \pi^0 e^+ \nu$ measurement, suppressing decay-in-flight (DIF) backgrounds, and suppressing the $\pi \rightarrow \mu \rightarrow e$ ``Michel'' decay chain  (four orders of magnitude more likely than the rare  $\pi \rightarrow e \nu$ process). Ultimately, it is expected that the ATAR will be able to suppress the muon decay positrons sufficiently, so that the low energy fraction of $\pi \rightarrow e \nu$ events extending below the \unit[52]{MeV} maximum Michel energy can be directly measured, greatly improving knowledge of ``low energy tail'',  the principal systematic uncertainty in previous measurements of $R_{e/\mu}$, to the level $<0.01\%$. In initial studies,  using simulated ATAR data and machine learning analysis techniques, has shown that suppression of the DIF background to the required level is feasible.

A highly segmented active target (\atar)~\cite{Mazza:2021adt} is a key new feature of the proposed PIONEER experiment. Relative to previous experiments, the use of \atar allows for discrimination against backgrounds by looking for deposition patterns internal to the target that are associated with the various signals' decay topologies.
%;  technical details and alternative designs of the sub-detector can be found in Appendix~\ref{sec:ATAR_appendix} with a detailed timeline described in Appendix~\ref{sec:ATAR_timeline_app}. 
The \atar\ will define the fiducial pion stop region, provide high resolution timing information,
%suppress decay in flight, suppress the $\pi \rightarrow \mu \rightarrow e$ Michel chain, which is four orders of magnitude more likely than the rare $\pi_{2e}$ process $\pi \rightarrow e \nu$,
and will furnish selective event triggers. Examples of event displays for \pie\ and \pme\ events are shown in Fig.~\ref{fig:Event_display}.

\begin{figure}[htbp]
\centering
% \includegraphics[width=0.8\textwidth]{Figures/event_display.png}
\vspace{-20mm}
\includegraphics[width=0.9\textwidth]{Figures/Simulation/event_display1_vt.pdf}
\caption{Simulated example displays of pion decay events in the \atar. Pions enter horizontally from the left; the  red dotted lines show the positions of the pion stops.
%and the green dotted lines show the position of positron exiting the ATAR.
The color of the bars indicates the deposited energy. Left column: X-Z (top) and Y-Z (bottom) strip  views of a \pie\ event.  Right column: Same views of a \pme\ event. The  blue dotted line shows the position of the decay muon stop.}
\label{fig:Event_display}
\end{figure}



For the measurement of the calorimeter response to \pie\ decays,  the \atar\  will suppress the $\pi \rightarrow \mu \rightarrow e$ decay at rest (\pdar), and pion and muon decay-in-flight (DIF)  low energy  backgrounds.
DAR events are identified by a good pulse pair resolution observing the \tmu\ $\pi\to\mu$ decay, and a tight positron observation window of about one pion lifetime.  \pdif\ events are  identified  by kinks in the trajectories, \dedx measurements along the track, and observed range in the target. %Examples of simulated event types are shown in Fig.~\ref{fig:EventTypes}.
%The low energy background (less than 52 MeV) will be suppressed %sufficiently so that the low energy tail of the calorimeter %\pie~ response  can be directly measured.
Furthermore, the \atar\ will suppress accidental muon stops that precede the trigger signal; these were a significant source of pile-up background in the previous experiments. 
Confirmation that  the observed positron belongs to the pion stopping vertex will also be obtained using tracking in the \atar\ and in additional tracking detectors (discussed in Sec.~\ref{sec:positron_detectors}).

To fulfill these goals the \atar\ must be able to detect both the exiting $e^+$, a minimum ionizing particle (MIP), and larger ($\thicksim$100 MIPs) energy deposits from $\pi^+$ and $\mu^+$.
The large dynamic range O(2000) of the signals is a significant challenge for the readout electronics  in the amplification and digitization stages.
The position of the energy deposits needs to be identified with sufficient granularity along the beam direction and in the transverse plane.
Furthermore, to identify single components of the decay processes a \SI{\sim 1.5}{\ns} pulse pair resolution is needed.

The \atar\ tentative design dimensions are 2$\times$2\,\si{\cm\squared} transverse to the beam. In the beam direction individual silicon sensors are tightly stacked with a total thickness of \SI{\sim 6}{\mm}.
%The requirement of avoiding dead material in the detector volume precludes the use of bump bonded electronics readout chips.
A strip geometry with the electronic readout connected on the side of the active region via wire bonding is foreseen.
The strips are oriented at \ang{90} to each other in subsequent staggered planes to provide measurement of both coordinates of interest and to allow space for the readout and wire bonds.
The preliminary sensor geometry has strips with a pitch of \SI{200}{\micro\metre}, so that a sensor would have 100 strips mated to a chip with 100 channels and \SI{2}{\cm} width, a standard dimension for microchips. 
A best estimate at present for the sensor thickness is around \SI{120}{\micro\metre} to avoid support structures for the sensor, which would introduce dead area. 
To reach a total thickness of about \SI{6}{\mm}, $\thicksim$50 planes are needed, so in total the \atar\  would comprise $\thicksim$5000 channels.
The detectors are paired with the high-voltage facing each other in a pair to avoid ground and high voltage in proximity. 
In the preliminary design, shown in Fig.~\ref{fig:ATAR_scheme}, the strips are wire bonded, with a connection alternating on the four sides, to a flex that brings the signal to a readout chip positioned a few cm away from the active volume.
This removes the chip from the path of the exiting positrons, reducing its degradation of their energy resolution.
The flex will be produced with aluminium traces so that the cable material per flex would be \SI{\sim 0.025}{g/\cm\squared}. 
In the figures in this proposal, all cables are shown exiting downstream.
A readout from both ends is being investigated to reduce the average material traversed by exiting positrons. 
At present, the maximum material in the path of the positrons occurs when 12 flexes are traversed. 
The readout ASIC sits on the first flex that tapers out to accommodate the additional traces. 
Then the flex is connected, via connector, to a PCB connected to a second flex that brings the amplified signal to the digitizers in the back end.
%Alternative detector designs that are being pursued are discussed in Appendix~\ref{sec:ATAR_mech_app}.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.4\textwidth]{Figures/ATAR.png}
\includegraphics[width=0.55\textwidth]{Figures/ATAR_scheme_2.png}
\caption{Left: \atar\ position in the beam line. Right: Concept schematic design of the \atar. The flex from the first, third and fifth sensors is directed in and out of the page. The modules are attached on the HV side and with a few  \si{\micro\metre} of separation on the strip side. 48 sensors are coupled in 24 pairs. }
\label{fig:ATAR_scheme}
\end{figure}

The chosen technology for the \atar\ is Low Gain Avalanche Detector (LGAD)~\cite{bib:LGAD}, 
%(detailed description in Appendix~\ref{sec:LGAD_app}), 
thin silicon detectors with moderate internal gain.
A \SI{120}{\micro\metre} thick LGAD sensor, coupled to fast electronics, has a time resolution of less than \SI{100}{\ps} on the rising edge and can separate a single hit from two overlapping hits if they arrive more than \SI{1.5}{\ns} apart.
Preliminary studies made with X-rays coming from the Stanford light source (SSRL)~\cite{GALLOWAY20195} and PSI~\cite{Andra:ay5534} show that LGADs have an energy resolution of around \SI{10}{\percent}.
%; more detailed results are reported in Appendix~\ref{sec:LGAD_app}.
The effect of gain saturation that was reported in the community in the past year~\cite{gainsuppr} also needs to be studied.
The LGAD technology was chosen over standard silicon technology because of the intrinsic gain and thin bulk. 
Normal silicon detectors without gain need 300--500\,\si{\micro\metre} of active silicon to have enough collected charge for high MIP detection efficiency.  This would degrade granularity in the beam direction, time resolution and pulse separation discrimination. 
%A brief discussion on alternative technologies is presented in Appendix~\ref{sec:LGAD_app}.

Current standard LGADs have a limitation in terms of granularity and active area. To achieve a \SI{\sim 100}{\percent}  active area several technologies still at prototype level are being evaluated for \nexp, such as AC-LGADs~\cite{Apresyan:2020ipp} and TL-LGADs~\cite{9081916}. 
%Studies were made on strip AC-LGAD prototypes from BNL as shown in Appendix~\ref{sec:ACLGAD_app}.
%Results on sensor simulation  are also reported in Appendix~\ref{sec:ACLGAD_app} and
%additional LGAD technologies are being evaluated as reported in Appendix~\ref{sec:TILGAD_app}.

\subsubsection{AC-LGADs}
\label{sec:ACLGAD_app}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.4\textwidth]{Figures/sensor.png}
\includegraphics[width=0.5\textwidth]{Figures/FNAL_TB.png}
\caption{Left: prototype BNL AC-LGAD strip sensor with 80\,$\mu$m wide strips and pitch of (left to right) 100, 150, 200\,$\mu$m. Right: sensor response ($P_{max}$) as a function of position (perpendicular to the strip) of two strips with 200~$\mu m$ of pitch~\cite{ACLGADpico}. The dashed lines highlight the position of the two strips in the plot. Data taken at the FNAL 120\,GeV proton test beam facility.}
\label{fig:FNAL_data}
\end{figure}

AC-LGADs overcome the granularity limitation of traditional LGADs and have been shown to provide spatial resolution of the order of tens of $\mu$m~\cite{Tornago:2020otn}. AC-LGAD design also allows to have a completely active sensor with no dead regions.
Studies were conducted on strip AC-LGAD prototypes from Brookhaven National Lab (BNL) (Fig.~\ref{fig:FNAL_data}, Left). 
The sensors have been tested with a laboratory IR laser TCT station~\cite{Particulars} and at a Fermilab (FNAL) test beam~\cite{ACLGADpico}.
The response of two strips of a 200\,$\mu$m pitch BNL AC-LGAD as a function of position can be seen in Fig.~\ref{fig:FNAL_data} (Right). The position resolution of this prototype sensor varies between 5-15~$\mu m$ in the direction perpendicular to the strip.
In the next few years several prototypes will be tested in laboratories and test beams to identify the right parameter configuration, then a PIONEER-specific production will be made at Brookhaven.

The envisioned metal size for the 200\,$\mu$m pitch strips, as well as other parameters of interest for the sensor such as the doping profile, needs to be confirmed after a testing R\&D campaign and TCAD simulations. 
These parameters have been studied with the TCAD Silvaco \cite{Silvaco} to have a good representation of the observed sensor performance. Simulations with TCAD software are important to compare with existing prototype data and to help in optimizing the design, currently the simulated sensor response show a reasonably good match with FNAL TB data. 
Studies made with simulations tools will provide crucial input for the future PIONEER sensor production.
%Figure~\ref{fig:simulation} (Left) shows the simulated waveforms of four metal pads using TCAD Silvaco 
%Figure~\ref{fig:simulation} (Right) is the Pmax profile of 200\,$\mu$m pitch strip sensors with different sheet resistivity and the same geometry of the BNL strip prototype already introduced. 500\,$\Omega$ shows a reasonably good match with FNAL TB data.
%These simulations are for 50\,$\mu$m thick sensors, to simulate the final PIONEER prototype they need to be redone for 120\,$\mu$m of thickness.

%\iffalse
%\begin{figure}[htbp]
%\centering
%\includegraphics[width=0.4\textwidth]{Figures/Simulation.png}
%\includegraphics[width=0.55\textwidth]{Figures/PmaxSim.png}
%\caption{Left: AC-LGAD strip simulated waveform with TCAD Silvaco. The sensor is a 200\,$\mu$m pitch strip sensors with N+ sheet resistivity of 500\,$\Omega$. Right: Pulse maximum (normalized) as a function of position for a strip with 80\,$\mu$m width and 200\,$\mu$m pitch. Left edge of the plot is the center of the readout strip. Curves are for data (FNAL testbeam) and TCAD Silvaco simulation with several N+ sheet resistivity. }
%\label{fig:simulation}
%\end{figure}
%\fi


\subsubsection{TI-LGADs}
\label{sec:TILGAD_app}
Trench Isolated (TI) LGADs are a novel silicon sensor technology that utilizes a deep narrow trench to electrically isolate neighboring pixels to prevent breakdown, as opposed to standard LGADs which use a junction termination extension to prevent breakdown at the pixel edges \cite{9081916}. By utilizing the deep trench isolation technology, the no-gain region is reduced to a few micrometers, thus achieving a higher fill factor than regular LGADs. 
Prototypes TI-LGADs sensors from Fondazione Bruno Kessler (FBK) \cite{9081916} were studied at UCSC.
TI-LGADs show the standard response of a conventional LGAD and exhibits a small amount of “cross-talk”. Furthermore the response of the sensor is constant along the strip.
The maximum values of the pulse shape for the neighbor strips correspond to ~3$\%$ of the maximum value of the red pulse showing there is good isolation between strips.
New TI-LGADs productions are envisioned at FBK and other vendors, the prototypes will be tested in laboratories and test beams to find a suitable alternative sensor technology for PIONEER.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Electronics and readout chain}
\label{sec:ATAR_electronics_app}

To read out the ATAR sensors, two crucial electronic components need to be identified: an amplifier chip and a digitizer board.
%The ASIC sits on the flex connected to the sensor with several centimeters of separation.
The ASIC needs to be fast enough for the sensor in use; for the signal rise time in the 120\,$\mu$m-thick prototype sensors,  a bandwidth of 1\,GHz should be sufficient.
However, the high dynamic range (2000) requirement for the ATAR brings major complications to the readout.
Current fast readout chips usually have a dynamic range of $<$~1000, since they are targeted at MIPs-only detection in tracker sub-systems.
One possibility is to develop an amplifier chip with logarithmic response or dynamic gain switching as well as a high enough bandwidth, currently no such chip exists with the necessary characteristics.
Already available integrated chips, such as FAST~\cite{OLAVE2021164615} and FAST2, are being evaluated.
Some new ASIC technologies that are being developed at UCSC in collaboration with external companies can run with 2.5V maximum signal, this allows for an increased dynamic range.

Since the amplification chip has to be positioned away from the active region, the effect of placing a short (5\,cm) flex cable between the sensor and the amplification stage has to be studied.
To study this a prototype flex was produced and the effect on LGAD signals will be studied.

To successfully reconstruct the decay chains, the ATAR is expected to be fully digitized at each event.
To achieve this goal, a high bandwidth digitizer with sufficient bandwidth and sampling rate have to be identified. 
The same issue afflicting the amplifier, the high dynamic range, is also problematic for the digitization stage. 
A digitizer that would suit PIONEER's requirements needs to be identified, a ready commercial solution would be the best option but the cost per channel might be prohibitive. 
For this reason the collaboration is exploring the possibility to develop a new kind of digitizer specific to this application.

\subsubsection{ATAR0 prototype}
\label{sec:ATAR0}
A first ATAR demonstrator (ATAR0) is foreseen with available sensor prototypes: the current BNL AC-LGAD production has 2.5~cm long strips with a pitch of 500~$\mu$m, which is close to the final 200~$\mu$m 2x2~cm$^2$ ATAR design (however the sensor thickness is 50~$\mu$m instead of the final design 120~$\mu$m). Since a 50~$\mu$m thick sensor is fabricated on a support wafer of a few 100s $\mu$m, the devices would need to undergo an etching procedure to have full active volume, the thinning procedure can be executed at BNL. The BNL sensor group has experience with wafer lapping and chemical mechanical planarization (CMP). The sensor would be initially lapped to remove most of the thickness of the handling thick substrate, followed by CMP for final polish. The etching rate would be determined on dummy wafers and the process would be optimized to reach the required final thickness.
The prototype would have a few layers (5-10) with a reduced number of channels to detect the temporal development of a muon or pion decay. As the layers would need to be very close to each other, a suitable readout board needs to be developed. The board might be built with discrete components or using a chip such as FAST2.
The prototype would be then tested in a pion/muon beamline either at TRIUMF or a PSI. Hopefully such a prototype can be produced by the end of 2023.


%To read out the \atar\ sensors two crucial electronic components need to be identified: an amplifier chip and a digitization board.
%Preliminary tests on  available solutions are reported in Appendix~\ref{sec:ATAR_electronics_app}. 
%The amplifier chip needs to be fast enough for the sensor in use, since the prototype sensors are 120~$\mu m$ thick a bandwidth of 1~GHz should be sufficient.
%Since the amplification chip has to be positioned away from active region, the effect of placing a short (\SI{5}{\cm}) flex cable between the sensor and the amplification stage will be studied.
%To successfully reconstruct the decay chains the \atar\ is expected to be fully digitized at each triggered event. 
%The fast charge collection time of thin LGADs will allow separation of subsequent charge depositions as mentioned before.  % by using advanced de-convolution algorithms.  
%To achieve this goal a high bandwidth digitizer with sufficient sampling rate has to be used. 
%A discussion on  available amplifier chips and digitizers is reported in Appendix~\ref{sec:ATAR_electronics_app}. 



==> PioneerExperiment/ATAR/positron_detectors.tex <==
\label{sec:positron_detectors}
A dual layer cylindrical silicon strip tracker is situated between the \atar\ and the calorimeter to measure the  positron position in two dimensions (along the beam direction, $z$, and azimuthal angle, $\phi$), and time, as indicated in Fig.~\ref{fig:atar}.
The detector has  an inner diameter of \SI{5}{\cm} and a length of \SI{25}{\cm}. 
%To avoid energy degradation the tracker has to be thin, without dead material and fairly homogeneous.
%Silicon strip sensors would be the right technology for the tracker. 
The readout ASIC will be wire bonded at a location outside  the calorimeter active solid angle.
Overlapping lengths of long strips (about \SI{10}{\cm}) are needed to cover the entire region.


Two layers of strips with a small stereo angle  between them will provide % X-Y hit position,
O(mm) $z$ resolution and \SI{300}{\micro\metre} resolution in the direction perpendicular to the strips.
An alternative under consideration is to connect  two or three strip sensors in a line reading out both ends to obtain O(mm) position information along the strip position using charge attenuation information.
%similar to the ATAR technique shown in Fig.~\ref{fig:double_side} (Left).

The silicon strip sensors may be constructed with  either regular silicon or LGADs. %depending on the time resolution requirements and energy degradation.
Regular silicon would have \SI{\sim 300}{\micro\metre} of thickness for positron detection with a time resolution \SI{< 1}{\ns}, while LGADs can be \SI{50}{\micro\metre} or less with a time resolution of \SI{< 50}{\ps}.
However, LGAD silicon strips with length of 10\,cm present an additional challenge
%to the ATAR 2~cm long strips, 
while for the ATLAS detector standard silicon strips with \SI{\sim 10}{\cm} of length have been successfully fabricated on 8-inch wafers \cite{CERN-LHCC-2017-005}.

==> PioneerExperiment/Beam/beam1.tex <==


The basic beam requirements for PIONEER are summarized in Table~\ref{tab:beam}. The values given are initial estimates, and some of the requirements,
e.g. in the longitudinal and transverse beam extent, might be relaxed pending further studies.
In the following we will only discuss PIONEER Phase I beam requirements, but the parameters for the full experimental program are also considered.

%should be kept in mind,
%so that they are respected in the design of most expensive detector components (i.e. the CALO) and remain consistent with available PSI beams.  

\begin{table}[htb]
\centering
\begin{tabular}{ccccccc}
\toprule
Phase & p  & $\Delta$p/p & $\Delta$Z 	& $\Delta$X x $\Delta$Y& $\Delta$X',$\Delta$Y'  & R$_\pi$ \\ 
      & (MeV/c) & (\%) & (mm) 				& (mm$^2)$ 				& 						 & (10$^6$/s) \\ 
\hline 
I & 55-70 & 2 & 1 & 10x10 &  $\pm$10\degree & 0.3 \\ 
II,III & \app\ 85 & $\le$ 5 & 3 & 15x15 & $\pm$10\degree  & 20 \\ 
\bottomrule 
\end{tabular} 
\caption{Required beam properties. $\Delta$Z and $\Delta$X $\times$ $\Delta$Y are longitudinal (FWHM) range width and transverse (FWHM) beam sizes at target location, respectively.}
\label{tab:beam}
\vspace{-0mm}
\end{table}

The 0.01\% precision goal of the \remu\ measurement places stringent requirements on the  beam and target as discussed below. 
\bl 
\ListProperties(Margin=1cm, Hang1=true,Hide2=0,Numbers1=r,Numbers2=r,Progressive*=.5 cm,Start1=1)
& Pion stops: The efficiency for
detecting the $\pi-\mu$ sequence should be the same as for a $\pi$ stop; thus all decay muons must be  fully contained in  \atar. 
This drives the requirement for the small longitudinal and lateral size of the stopped $\pi$ distribution. Upstream  detectors (if necessary) will  be minimized, as they
increase the beam spot by scattering. 

& Positron detection: The \atar\ should  be small to reduce the positron energy deposited in it, though largely this loss can be reconstructed. The constraint on the beam entrance divergence is necessary to keep the  opening angle of the beam entrance cone
to 10\degree\ relative to its axis. (A larger cone will decrease the solid angle for positron detection and, in particular,  increase the surface for shower leakage.) This requirement limits the phase space acceptance to 175 $\pi\,$cm$\,$mrad.
%, which is not a problem for Phase I, but needs more careful considerations for Phase II. 
\el

\begin{figure}[htb]
\centering
\includegraphics[width=1\textwidth]{Figures/Beam/target.png}
\caption{Beam counters and \atar. An active degrader disk (not shown) is optional, and only required for p$>$55 MeV/c. The beam detectors systems LGAD1 and LGAD2 provide an event by event trajectory for entering particles.  It is conceivable that they can be rotated out of the beam for production running at the lowest operating momenta.}
\label{fig:atar}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\textwidth]{Figures/Beam/r-t.pdf}
\caption{ Range-energy (left) and  momentum-energy (right) relations for pions and muons. Muons from \pdar\ have 4.12 MeV kinetic energy and travel 
%\app 
0.8 mm in Si.}
\label{fig:r-p}
\end{figure}

Figure~\ref{fig:atar} sketches the baseline set-up for the beam-target section of the experiment. For a more complete description of the overall \atar-\calo\ design we refer
to Sec.~\ref{sect:Mech-Eng}.
%
Pions selected by an E$\times$B separator pass through a beam window of $70\,\mu$m Mylar, two LGAD detector planes (two crossed layers of $50\,\mu$m thick AC LGADS, each, denoted as BEAM in this proposal)
%, and a $70\,\mu$m thick Mylar vacuum entrance window 
to stop in the ATAR. %Optionally, a Be degrader disk can be inserted, but that is not 
No degrader or upsteam LGAD detectors may be necessary if a
suitable beam at p=55\,MeV/$c$ can be established. 
%(Optionally, a  conical beam halo scintillator can be inserted (not shown) as a degrader.) 
As sufficient beam intensity is expected, the beam spot may be improved by
collimation just upstream of the detector entrance. Collimators would also serve to suppress muons and electrons displaced by the angular deflection in the separator but
their design has to be carefully optimized between the competing requirements of collimating close to the target focus while absorbing positrons and gammas before they reach the
\calo. Some important aspects of the stopping beam can be understood from the pion range-energy relations shown in Fig.~\ref{fig:r-p}.\footnote{These were
calculated by SRIM (http://www.srim.org/) to describe the  slowing down of particles at low energies.}. 

A momentum of 55\,MeV/$c$ has several advantages including that the separator will work more efficiently
%, only minimal upstream degradation, naturally provided by the \beam\ detectors, is required
and a range width $\Delta Z$ of less than 0.4\,mm is expected for a 2\% $\Delta$p/p beam momentum acceptance. (The stopping range width would increase to 0.8\,mm at 70\,MeV/$c$.)
%and require the Be degrader.
The range-energy curve also shows how the separation between pions and muons of the same energy improves with the energy deposited in \atar.
%In that respect,
%a slightly higher momentum of 60\,MeV/$c$ may be advantageous. Then the range difference increases to 1\,mm, which augmented with dE/dx information,
%should highly suppress muons. %if ATAR reaches a few percent energy resolution.





==> PioneerExperiment/Beam/beam2.tex <==
The PSI High Intensity Proton Accelerator (HIPA) chain consists of a Cockcroft-Walton pre-accelerator, delivering 870\,keV protons to a set of two isochronous cyclotrons which further accelerate to the maximum 590\,MeV. 
In the Ring cyclotron, the protons are accelerated by four copper resonator cavities operated in continuous wave (CW) mode at a frequency of 50.6 MHz, giving the periodic 19.75\,ns beam microstructure and their final energy of 590\,MeV.
The $\pi$E5 channel is a high-intensity low-energy muon and pion beamline, with a maximum momentum of 120\,MeV/$c$, that views the second graphite production target, Target~E, at 165$^{\circ}$ with respect to the proton beam axis.
The $\pi$E5 channel is used exclusively for particle physics experiments, and is currently home to the MEG~II and Mu3e experiments.
The channel length from Target~E to end of the QSB43 quadrupole magnet and the entrance to the experimental area is 13\,m, giving approximately 7\,m of free space between the concrete wall and current MEG~II infrastructure.
In this area the SEP41 E$\times$B Wien Filter for particle separation, QSK quadrupole triplet for focusing the beam on the \atar\, and the PIONEER installation could be placed.
\begin{figure}[h]
	\centering
	\includegraphics[width=1\linewidth]{Figures/G4BLSIM_PiE5_Labeled.png}
	\caption{The \gbl\ model of the $\pi$E5 beamline including a stand-in calorimeter.}
	\label{fig:g4blsim_pie5_labeled}
\end{figure}

==> PioneerExperiment/Beam/beam3.tex <==


Simulations for both pion production at Target~E and transport of particles down the $\pi$E5 channel were performed using the \gbl\ toolkit ~\cite{Roberts:2008zzc}.
A figure of the $\pi$E5 beamline from the \gbl\ simulation, beginning at Target E and ending at the PIONEER calorimeter, is shown in Fig.~\ref{fig:g4blsim_pie5_labeled}.
The pion production simulation utilizes the parameterized cross sections developed for the High Intensity Muon Beamline (HiMB) project \cite{PhysRevAccelBeams.19.024701}.
All simulation results are scaled to the nominal 2.2~mA proton beam current at PSI.

The \gbl\ simulation was originally tuned for 28\,MeV/$c$ muons and has been rescaled for the respective pion momenta.
Some additional tuning was performed for the last two dipoles and quadrupole triplets to optimize transmission through the SEP41 and on to the \atar.
The physical volume of the SEP41 is included but its electric and magnetic fields are not enabled for these simulations.
Rates for pions and muons reaching the entrance to the experimental area (QSB43) and 4.8\,m downstream at the center of the calorimeter volume (\calo\ center) for beamline central momenta ranging from 55 to 75\,MeV/$c$ are shown in Fig.~\ref{fig:piE5rates}.
The rates for those particles at the lower and upper end of the possible momentum ranges are listed in Table~\ref{tbl:rates}.
The pion rates calculated in the simulation at the center of the calorimeter for a 2\% momentum-bite 
are sufficient for the \remu\ measurement planned in Phase I of PIONEER, even when
further losses in the SEP41 or upstream collimation, necessary for reducing background events in the \atar\ and calorimeter, are included.
For PIONEER Phase II, III increasing the momentum and the momentum bite will be required.



\begin{figure}[htb]
	\centering
	\includegraphics[width=.8\linewidth]{Figures/PiE5_Rates.pdf}
	\caption{The rates for pions and muons at the entrance to the experimental area (QSB43) and reaching the center of the calorimeter, calculated in the $\pi$E5 \gbl\ simulation.}
	\label{fig:piE5rates}
\end{figure}

\begin{center}
\begin{table}
\begin{tabular}{p{4cm}|p{2cm}<{\centering}|p{2cm}<{\centering}|
                p{2cm}<{\centering}}
    \toprule
	Beamline Position& $p_{\pi}$ (MeV/$c$) & $\pi^{+}$ Rate&$\mu^{+}$ Rate \\
	\hline
	QSB43           & 55 & 6.3 & 12.3 \\
	\calo\ Center   & 55 & 1.0 & 6.1 \\
	\hline
	QSB43           & 75 & 61.5 & 30.2 \\
	\calo\ Center   & 75 & 11.1 & 15.1 \\
	\bottomrule
\end{tabular}
\caption{Particle Rates ($\times 10^{6}$ $s^{-1}$) in $\pi$E5 for a 2\% momentum-bite calculated in the \gbl\ simulation. 
%At the center of the calorimeter, the lower pion rates at 55\,MeV/$c$ fall below the requirements for the experiment, whereas at 75\,MeV/$c$ the rate exceeds the requirements.
}\vspace{-3mm}
%	\end{table}
\label{tbl:rates}
\end{table}
\end{center}
A very preliminary study to focus the beam onto the calorimeter center positions by simulating 65~MeV/c pions with their decay disabled is displayed in Fig.~\ref{fig:phasespace}. The horizontal ($x-x^{\prime}$) phase space indicates a pronounced non-Gaussian nature, while the vertical ($y-y^{\prime}$) phase space demonstrates a well defined focus. The complex structure of of the horizontal phase space emphasizes that full \gbl\
simulations are required to tune the beam and, in particular, experimental verification is indispensable to achieve the desired small beam spot 
on \atar. At the moment, there is no readily available experimental data that could verify our preliminary simulations for $\pi^+$ beams. The above used simulation code was verified so far using surface muon beams of 28 MeV/c momentum only. The last experiment using pion beams at $\pi$E5 was the PiHe experiment that needed high $\pi^-$ rates for pionic helium spectroscopy~\cite{Hori:2020iom}.


\begin{figure}[htb]
	\centering
	\subfloat{
    \includegraphics[width=0.4\textwidth,height=0.4\textwidth]{Figures/pions_XXp.png}}
    \qquad
    \subfloat{
    \includegraphics[width=0.4\textwidth,height=0.4\textwidth]{Figures/pions_YYp.png}}
	\caption{Preliminary pion phase space distributions at the \calo\ center position for 65~MeV/$c$ pions with decay disabled from the \gbl\ simulation of $\pi$E5. Left: Horizontal. Right: Vertical. The calculated emitance $\epsilon$ for each is included in the plot as text. The non-Gaussian structure of these phase spaces present a challenge in correctly modeling the beam transport.}
	\label{fig:phasespace}
\end{figure}

Key experimental parameters, including the design of the beam conduit into the calorimeter and the geometry of the \atar\, rely on a detailed understanding of the $\pi^+$ beam properties at $\pi$E5 at the targeted momentum range (55-75\,MeV/$c$).  
The most important parameters to be determined are the $\pi^+ / \mu^+ / e^+$ rates as a function of beam momentum, the momentum bite $\Delta p/p$, the final focus and the capability to select a clean $\pi^+$ beam by applying a Wien (E$\times$B) filter.
 Measurements of available $\pi^{+}$ rates and comparison to simulation will be performed \textcolor{red}{in 2022 to determine} achievable pion rates at the \atar.
%For this purpose we propose to carry out detailed measurement program of the $\pi$E5 pion beam at PSI, adapting SiPM-based beamline instrumentation that was used to characterize pion and muon rates in the past. Because
%of their urgency in informing the detector design we request a first study in 2022 (beam request submitted separately). 


%In this experiment, with the momentum slit fully opened ($\delta p/p \approx 0.08$ FWHM) and no separation, a pion rate of $R_{\pi} = 1.38 \cdot 10^8$ Hz and a beam content of  79\% $e^-$, 18\% $\pi^-$, 3$\mu^-$ was estimated from measurements. 
%By applying the strongest available separator at PSI (voltages at $\pm$ 275 kV), $R_{\pi} = 3.5 \cdot 10^7$, $\sim$45 mrad separation of the pion and electron beam was achieved, which improved the electrons to pion ratio to  $\sim$0.1 near the target position. However, these results did not match either the expected values.









==> PioneerExperiment/BeamSim.tex <==
\subsection{Beamline Simulations}
	
\subsubsection{Beamline Simulations and Optimization}
The PSI High Intensity Proton Accelerator (HIPA) chain consists of a Cockcroft-Walton pre-accelerator, delivering 870 keV protons to a set of two isochronous cyclotrons which further accelerate to the maximum 590 MeV. 
In the Ring cyclotron, the protons are accelerated by four copper resonator cavities operated in continuous wave (CW) mode at a frequency of 50.6 MHz, giving the periodic 19.75~ns beam microstructure and their final energy of 590 MeV.
The $\pi$E5 channel is a high-intensity low-energy muon and pion beamline, with a maximum momentum of 120~MeV/c, that views the second graphite production target, Target~E, at 165$^{\circ}$ with respect to the proton beam axis.
The $\pi$E5 channel is used exclusively for particle physics experiments, and is currently home to the MEG~II and Mu3e experiments.
The channel length from Target~E to end of the QSB43 quadrupole magnet and the entrance to the experimental area is 13~m, giving approximately 7~m of free space between the concrete wall and current MEG~II infrastructure.
In this area the SEP41 E$\times$B Wien Filter for particle separation, QSK quadrupole triplet for focusing the beam on the ATAR, and the PIONEER installation could be placed.
\begin{figure}[h]
	\centering
	\includegraphics[width=1\linewidth]{Figures/G4BLSIM_PiE5_Labeled.png}
	\caption{The G4beamline model of the $\pi$E5 beamline including a stand-in calorimeter. Important elements along the beamline where rates are compared are labeled.}
	\label{fig:g4blsim_pie5_labeled}
\end{figure}

Simulations for both pion production at Target~E and transport of particles down the $\pi$E5 channel are performed using the G4Beamline toolkit~\cite{Roberts:2008zzc}.
A figure of the $\pi$E5 beamline from the G4Beamline simulation, beginning at Target E and ending at the PIONEER calorimeter, is shown in \cref{fig:g4blsim_pie5_labeled}.
The pion production simulation utilizes the parameterized cross section developed for the High Intensity Muon Beamline (HiMB) project.
The absolute rates determined from the simulation for particles near the production target are shown in \cref{fig:productionrates}.
\begin{figure}[h]
	\centering
	\includegraphics[width=1\linewidth]{Figures/TgEProdSim_HiMBHYBRID_10B-PoT_MomSpecFromTarget_SF100_positive.pdf}
	\caption{The rates of positive charged particles produced at Target E with longitudinal momentum in the direction of the $\pi$E5 channel. }
	\label{fig:productionrates}
\end{figure}

The G4Beamline simulation was originally tuned for 28~MeV/c muons and has been rescaled for the respective pion momenta.
Some tuning was performed for the last two dipoles and quadrupole triplets to optimize transmission through the SEP41 and on to the ATAR.
Rates for pions and muons reaching the entrance to experimental area for beamline central momenta ranging from 55~MeV/c to 75~MeV/c are shown in \cref{fig:piE5rates}.
The rates for those particles reaching the entrance to the experimental area (QSB43) and 4.8~m downstream at the entrance to the calorimeter volume (CALO Entrance) at the lower and upper end of the possible momentum ranges are listed in \cref{tbl:rates_55MeVc} and \cref{tbl:rates_75MeVc}.  

\begin{figure}[h]
	\centering
	\includegraphics[width=1\linewidth]{Figures/AtQSB43DSPiE5_Rates_PionsMuons.png}
	\caption{The rates for pions and muons at the entrance to the experimental area (QSB43).}
	\label{fig:piE5rates}
\end{figure}

	\begin{center}
	\begin{tabular}{p{4cm}||p{3cm}|p{3cm}|p{3cm}} 
		\multicolumn{4}{c}{Particle Rates ($\times 10^{8}$) in $\pi$E5 (p$_{\pi^{+}}$=55 MeV/c) at 2.2~mA I$_{p}$} \\
		\hline
		Beamline Position& $\pi^{+}$ & $\mu^{+}$ & $e^{+}$\\
		\hline
		QSB43 & 0.50 & 1.22 & x\\
		CALO Entrance & 0.09 & 0.59 & x\\
	\end{tabular}
	\label{tbl:rates_55MeVc}
\end{center}

\begin{center}
	\begin{tabular}{p{4cm}||p{3cm}|p{3cm}|p{3cm}} 
		\multicolumn{4}{c}{Particle Rates ($\times 10^{8}$) in $\pi$E5 (p$_{\pi^{+}}$=75 MeV/c) at 2.2~mA I$_{p}$} \\
		\hline
		Beamline Position& $\pi^{+}$ & $\mu^{+}$ & $e^{+}$\\
		\hline
		QSB43 & 4.66 & 2.68 & x\\
		CALO Entrance & 1.10 & 1.34 & x\\
	\end{tabular}
    \label{tbl:rates_75MeVc}
\end{center}

The pion rates calculated in simulation at the entrance to the calorimeter are approximately a factor two lower than the latest measurements at $\pi$E5, nevertheless they exceed the requirements of the experiment by two orders of magnitude.
This high rate would allow for losses in the SEP41 or upstream collimation, necessary for reducing background events in the ATAR and calorimeter.
Verification of these rates from measurements and comparison to simulation will be critical in determining achievable pion rates at the ATAR.
\subsection{Beamline Studies}
	
	{\it AS: editing offline}

==> PioneerExperiment/Calorimeter/Calorimeter_Mech_Eng.tex <==





\label{sect:Mech-Eng}

\subsubsection*{Requirements}

Mechanical engineering considerations for the LXe calorimeter are discussed below.

\bl [itemize]
\ListProperties(Start1=1)
& The \calo\ mechanical design has to support a load of about 9 tons of LXe as well as
the required cryogenic envelope, consisting of a cold vessel and an insulation vacuum. Ideally, the heat load
of the new system should be compatible with existing MEG cooling and purification infrastructure. 
& The beam region consist of an entrance cone to focus a  beam with 10\degree\ divergence onto a beam spot of
about 1 cm$^2$. The entrance side will support the \beam\ detectors. The exit side should be in air, allow the
insertion of \atar\ and \track\ and their associated electronics, and provide sufficient heat removal.
& The \atar\ target region should be surrounded by thin beam pipes. The goal is to
minimize material in the \calo\ acceptance of close to degree=140\degree\ in polar angle, while covering
the full azimuth. 
& The \atar\ and \track\ region is very space limited, while increasing the inner pipe radii is problematic, both in terms
of solid angle and window strengths. A compromise between these conflicting requirements needs to be optimized.
& The PIONEER detector is designed for a measurement program extending over a decade. Both routine services as well as major
repairs and upgrades must be supported by the design.
\el

\subsubsection*{Conceptual design}


The calorimeter is built of interactive functional blocks incorporating a top load concept with the intent to be modular and to allow for ease of maintenance.  The functional blocks are described below and a drawing is shown in Figure~\ref{fig:LXe_Calo_XSec}.


%\begin{enumerate}
%%%%%%\item A vessel for liquid xenon.
%%%%%\item A spherical surface within the xenon to mount scintillation light detectors.
%%%%\item Thermal insulation for the liquid xenon.
%%%\item An airspace in the middle of the xenon for the target.
%\item A path for the beam to get to the target.
%\end{enumerate}
%
%Through several iterations these general functional blocks were refined to a modular top loading concept. \\

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.8\textwidth]{Figures/LXe Calorimeter XSec04.png}
	\caption{Concept design of the liquid xenon calorimeter.  For scale, the lid is 3.05 m diameter. The yellow circles are merely representative of the photosensors; they are not placed accurately.}
	\label{fig:LXe_Calo_XSec}
\end{figure}

\ListProperties(Start1=1)
\textbf{1. Liquid xenon vessel}:
This vessel has a spherical bottom to follow the contour of the detector mounting surface. This both reduces bending stress in the walls and reduces the volume of xenon required to cover the detectors.  Running through this vessel horizontally is a cone-tube pathway.  The tube portion, which surrounds the target, is envisioned as beryllium. The cone may be of a variety of metals.  The connection between the two components is designed to be a braze or weld.

\textbf{2. Detector mounting surface}:
Beyond the basic requirement of being spherical and holding detectors, the inner radius is set at 0.9\,m to achieve the required number of radiation lengths of xenon.

\textbf{3. Thermal insulation}:
To achieve the best insulation, the calorimeter has been designed to be a vacuum dewar.  The support of the liquid xenon vessel is achieved by hanging it on turnbuckles made of material which does not conduct heat well.  Stainless steel is seen as the most likely option.  If additional reduction in heat load is needed the link could be changed to titanium, allowing for a reduced cross section.  The more complicated portion of the thermal insulation is maintaining vacuum around the incoming beam and the target space.  This is made easier by having a break in this tube.  The beam tube loads from one side, the target tube from the other.  Both terminate in thin vacuum barrier windows which allow beam passage.  To accommodate both temperature induced dimensional changes and deflection from weight loading, there are two bellows present.  The tube running through the xenon vessel has bellows on the target loading side.  There is a large bellows on the top of the  xenon vessel to allow cabling and piping to pass through the vacuum space.

\textbf{4. Target air space}:
The tube the target resides in is envisioned as beryllium.  This tube is mounted on a flange on the vacuum vessel and protrudes past the centerline by approximately 175\,mm.  The inside end of the tube is capped with a window that allows passage of the beam and also acts as a vacuum barrier.  This tube also contains the tracking detector and the necessary cabling.  

\textbf{5. Beam path to the target}:
The beam is shown focusing with a center line to the beam edge angle of 10 degrees. % Designed for this beam focusing angle are two cones.  
The inner cone is between the beam (at atmospheric pressure) and the vacuum (insulation).  The outer cone is the barrier  between the vacuum and the xenon. Further studies might lead to a modification of the downstream exit pipe to mirror the entrance side, and the optimization of the ATAR holder,
to allow pass through of \pdif\ muons. 

==> PioneerExperiment/Calorimeter/Othercal.tex <==

A LYSO crystal calorimeter is also being investigated as an alternative to LXe; it would provide natural segmentation as in  the PEN/PiBETA experiments. We discuss this further in the Appendix.

==> PioneerExperiment/Calorimeter/Photosensors.tex <==


In order to readout the liquid xenon scintillation light, special photo sensors are necessary due to the short scintillation wavelength of 175\,nm and the low operation temperature of 165\,K. Two types of photo sensors were developed for this purpose by Hamamatsu K.K. and the MEG/MEG II collaboration: 2-inch photomultipliers (PMT) and multi-pixel photo sensors (MPPC).
A round-shaped 2-inch PMT sensitive to VUV light (R9869) has been developed using
Bialkali  (K-Cs-Sb) photocathode and a synthetic silica window. It achieved a quantum efficiency of \SI{15}{\percent}. Aluminum strips were added in the photocathode to prevent an increase of the sheet resistance at low temperature. 

In order to improve the granularity for the inner surface in the MEG-II experiment, a silicon photomultiplier, called MPPC (S10943-4372) with an active area of 12$\times$12\,mm$^{2}$, was developed. The main developments consisted in removing the protective layer, matching the optical properties of the silicon surface to that of the LXe, and reducing the thickness of the insensitive layer. Besides achieving higher granularity, there are several advantages to using SiPM with respect to photomultiplier tubes: they are insensitive to magnetic fields, the single photoelectron peak can be used for calibration of the sensor and the required supply voltage is relatively low (less than \SI{100}{\volt}).

However, as mentioned above, the PDE of the SiPMs were found to drastically decrease under exposure to the muon beam. Investigations are ongoing to understand the causes. It was however shown that the PDE could be recovered through an ``annealing'' procedure performed during the accelerator shutdown period. 
The gain of the PMTs was also found to decrease due to damage to the dynode induced by photoelectrons. The PMT lifetime is however sufficiently long and thus should not be of concern for PIONEER.

Considering the above, the baseline design for PIONEER is the use of PMTs on the outer surface targeting a coverage of \SI{20}{\percent} (1000~phototubes) of the surface. The choice of the photosensor technology might evolve depending on the developments regarding  SiPM performance degradation.

Simulations will be performed to study the impact on track identification capabilities and energy resolution  of adding SiPMs on the inner surface regions of the calorimeter. The ATAR is small (\SI{130}{\milli\meter}) 
and surrounded by a positron tracker which can measure the positron's incident position right before it enters the LXe calorimeter. In these conditions the addition of reflective material coatings on the inner surface may be sufficient for the PIONEER needs. However, it is notably difficult to accurately simulate UV optical properties on large scales. Agreement between data and photon transport simulations are sometimes poor, mainly because of the large number of optical interfaces, i.e., surfaces with a certain shape, absorbance and reflectance, that are not well known for the UV light from LXe (optical properties are indeed most often measured in vacuum). Apart from differences in refraction indices between vacuum and LXe, LXe may also alter the optical properties of some materials (e.g. \cite{Silva:2009ip, LZ:2015kxe, Neves:2016tcw}). It is thus particularly important to perform in-situ measurements in LXe to evaluate both the performance of SiPM in the LXe environment and deduce the appropriateness of surfaces for coatings (as well as possibly segmentation for pile-up rejection, see discussion in Sec.~\ref{sec:calo_simu}). For this purpose we have planned measurements at facilities where  LXe setups are  available.

%There are concerns in the PMT and MPPC in the MEG/MEG II experiment.
%The gain decrease of PMTs in MEG/MEG II experiment has been observed due to dynode material damaged by photoelectrons. The PMT life is however,  sufficiently long to sustain the MEG II whole period, and this may not be an issue for the PIONEER experiment.
%The PDE decrease of the MPPCs was observed in the MEG II experiment under the muon beam exposure. 
%The reason is still under investigation, but the PDE can be recovered by an "Annealing" procedure during the accelerator shutdown period which increases the temperature of the MPPCs. 

%The baseline design for the PIONEER photosensors uses PMTs on the outer surface because there is no magnetic field. The relatively large area in the outer surface should be covered but the perfromance is relatively insensitive to the  granularity.
%The SiPMs will be used if the degradation issues are overcome or only on the inner surfaces if that is shown to be necessary.


%The photosensor layout in the PIONEER experiment can be optimized because the detector shape is different from the MEG/MEG II experiment. The largest difference is the gamma/positron inner surface. In the PIONEER experiment, the inner surface will be very small, and it is under investigation whether photosensors on the inner surface are necessary or only putting some reflective material is sufficient.

==> PioneerExperiment/Calorimeter/caloverview.tex <==

\label{cal}

Due to its fast timing properties, high light yield with excellent energy resolution and highly uniform response, liquid xenon (LXe) 
read out by UV sensitive phototubes and state-of-the-art VUV SiPMs is considered for the calorimeter. Here, experience is drawn from the  MEG \cite{MEG:2016leq} and  MEG-II \cite{MEG:2018vi} experiments which use a large scale,  high rate  LXe detector to search for the lepton flavor violating muon decay, $\mu^+\rightarrow e^+ \gamma$.
 Experiments searching for the elusive dark matter (e.g. XENON, LUX-ZEPLIN) and (neutrinoless) double beta decay events (KamLAND-Zen, (n)EXO) also use detectors with similar scale liquid xenon cryostats. Unlike those latter experiments, MEG, like PIONEER, only detects scintillation light (other experiments rely on both scintillation and charge collection) and is a high rate experiment. In MEG, the rate of muon stops in the target was $\unit[3\times10^7]{\mu^+/s}$ and the LXe calorimeter rate due to photons was $\mathcal{O}$(\unit[0.3]{MHz}). The anticipated PIONEER calorimeter rate (due to  pion stop rate of 300\,kHz  in the ATAR for the $R_{e/\mu}$ measurement) is of the order handled by the  MEG LXe calorimeter. The main difference comes from the nature of the particles entering the calorimeter (gammas in the case of MEG and positrons for PIONEER) and the geometry  of the calorimeter leading to different event ``signatures''. The PIONEER LXe detector is foreseen to be a 25 radiation length, 3$\pi$~sr sphere surrounding the ATAR. A discussion on the capability of a large single volume to handle pileup events is given in Sec.~\ref{sec:calo_simu}.
 
 The homogeneity of the LXe detector is an advantage to reach high energy resolution which is important for determining accurately the low energy ``tail'' fraction of $\pi\rightarrow e \nu$ events. MEG  reported  an energy resolution of $\sigma=1.6\%$  which is expected to improve to 1.0\% for MEG-II for 50\,MeV gammas thanks to an improved read-out system using high-granularity SiPM detectors on the front face of the detector in place of photo-multipliers. The baseline energy resolution for PIONEER is 1.5\% similar to MEG's achieved resolution.
 
 The  energy resolution is impacted by the efficiency of collection of scintillation light which is itself influenced by design parameters (like photo-sensor coverage) and physical or technical parameters (like the light attenuation due to impurities in LXe, reflection of VUV light on surfaces, photo sensor refraction index, the level of dark current which impact the photo-electron threshold for summing the energies of the different photo-sensors, etc). In addition to the finite energy resolution of the calorimeter, photo-nuclear interactions, shower leakage and geometrical acceptance contribute to the low energy tail. The impact of photo-nuclear effects in LXe, for which little literature exists, will be determined by simulation and bench-marked against available data and new measurements. 
 
A GEANT-4 simulation of a bare LXe calorimeter geometry was used to determine the residual tail fraction below the Michel end point versus calorimeter depth for \pie~ events.  Figure~\ref{fig:tail_fraction}, Left, shows the energy deposited in the spherical calorimeter vs. the angle Theta with respect to the beam axis for a 25\,$X_0$ calorimeter depth.  Figure~\ref{fig:tail_fraction}, Right, shows the fraction of the energy deposited that is below  58\,MeV  vs. depth.  The volume of LXe required scales as the radius cubed and the required photo-sensor coverage scales as the radius squared.  These practical factors are optimized for smaller depth.  The containment of the shower slowly improves with increased depth.%, but it is a slow function.  
The depth was chosen to be 25\,$X_0$, which we use throughout this proposal.   
This choice, along with the spherical shape and $>\unit[3\pi]{sr}$ coverage, limits the effect of secondaries being missed by the calorimeter (e.g.~Bhabha scattered events) and will significantly reduce the contribution of shower leakage. We will continue to carefully model the calorimeter geometrical parameters and assess the expected detector sensitivity; see discussion in Sec.~\ref{sec:calo_simu}. 

Figure \ref{fig:resolution_scan} shows the energy spectrum for a 25\,$X_0$ calorimeter of varying intrinsic resolution; these results indicate that the tail correction is relatively insensitive to resolution. 
We are aiming for  resolution $\sigma=1.5\%$, based on the performance of the  MEG calorimeter. 

\begin{figure}[h!]
\centering
% \includegraphics[width=0.9\textwidth]{Figures/tail_fraction.png}
\includegraphics[width=0.9\textwidth]{Figures/Simulation/tail_fraction.pdf}
\caption{Left:  The energy deposited by monoenergetic 69.3\,MeV $e^{+}$ from \pie~ decays in a 25\,$X_0$ calorimeter with an energy resolution of 1.5\% vs. the angle Theta with respect to the beam axis.  The grey bands indicate the boundaries of the fiducial volume region (here, $30^{\circ}$).  Right: The shower tail fraction below 58\,MeV vs. the calorimeter depth in radiation lengths for the 69.3\,MeV $\pi \rightarrow e \nu$ events. 
%This does not include contributions from pion radiative decays.
%resolution of 1.5\% and a depth of $25\,X_0$.
}
\label{fig:tail_fraction}
\end{figure}

\begin{figure}[h!]
\centering
% \includegraphics[width=0.5\textwidth]{Figures/resolution_scan_25_X0.png}
\includegraphics[width=\textwidth]{Figures/Simulation/resolution_scan_25_x0_michel.pdf}
\caption{The effect of energy resolution on a 25\,$X_0$ calorimeter. The events indicated with a solid line are monoenergetic 69.3\,MeV $e^+$ from $\pi \rightarrow e \nu$ decay. The events indicated with a dashed line are the Michel spectrum from muon decay. The dashed grey line at 53 MeV represents the nominal endpoint of the Michel spectrum.
}
\label{fig:resolution_scan}
\end{figure}

 
 The xenon scintillation light absorption length has been  measured for MEG to be more than \unit[1]{m} \cite{Baldini:2004ph}.
 %which is highly advantageous when targeting a high energy resolution as is needed for PIONEER. 
 However, the light absorption length can be significantly reduced through absorption by impurities such as H$_2$O and O$_2$.
A large scale detector requires purification at the ppb level  which was achieved by MEG.
The purification system and the cryostat design (needed to maintain the xenon at \unit[165]{K} \cite{Mihara:2011zza}) of MEG will be considered for scaling up the design for PIONEER (see Sec.~\ref{sec:LXe_Cryogenics-purification}).
%, see section \ref{sec: LXe_photosensors}.

 MEG-II performed extensive R\&D in collaboration with Hamamatsu to develop large MPPC (Multi-Pixel Photon Counter) detectors ($12 \times$\SI{12}{\milli \meter \squared}) while maintaining optimal performance characteristics of  a small decay constant and good gain uniformity.
Efficient detection of VUV light requires careful choice of the silicon layer assembly and coatings. For their chosen sensor, the MEG-II collaboration reported a photon detection efficiency (PDE) of $\sim20\%$ \cite{MEG:2018vi} but observed later degradation of the PDE in LXe \cite{meg2sipm} which is under investigation. Below we discuss details of  photosensor options considered for PIONEER.

%Nevertheless, detailed studies need  to be done, in particular, because the geometry of the PIONEER and MEG detectors are different. However, the $\pi^+\to \pi^0 e^+ \nu (\gamma)$ measurement requires a rate of 10 MHz,
%an order of magnitude higher than the  PiBETA experiment which used a segmented crystal calorimeter. Detailed simulation studies are required to assess the capability of the 3$\pi$ sr PIONEER detector to handle pileup events in the high rate environment. 

==> PioneerExperiment/Calorimeter/cryogenics-purification.tex <==
\label{cryo-puri}

A system consisting of the following equipment is required in order to stabilize a large volume of liquid xenon in the detector:

\begin{enumerate}
\item High-pressure gas tanks for xenon storage,
\item Gas xenon purification system,
\item Liquid xenon purification system,
\item Refrigeration,
\item Temperature and pressure control system.
\end{enumerate}

Piping for transporting xenon either in the gas or liquid phase is required as appropriate. In addition to these, a cryostat that can temporarily hold xenon in a liquid state during emergencies or maintenance ensures efficient operation of the detector. \\

\ListProperties(Start1=1)
\textbf{1. High-pressure gas tanks for xenon storage}:
Xenon is stored in high-pressure gas tanks at room temperature during  detector maintenance periods. A storage tank that can withstand a pressure of 5.8 MPa at 17$^\mathrm{o}$C (1.1g/cm$^3$, the critical point of xenon) is required. After detector operation, the xenon is recovered in the storage tank by cooling the tank with liquid nitrogen. This requires a liquid nitrogen bath to cool the high-pressure gas tank.

\textbf{2. Gas xenon purification system}:
When operating the LXe detector, it is necessary to reduce the xenon gas pressure provided from the high-pressure tanks and then to remove impurities in the gas before filling in the detector cryostat. Metal-heated getter purifier technology has been used in previous experiments and will be employed also in the PIONEER experiment.

\textbf{3. Liquid Xenon Purification System}:
Based on the experience of the MEG experiment \cite{MEG:2016leq}, it is known that even if the xenon gas is liquefied in the detector after impurity removal by the gaseous-phase purification system, impurities remaining on the detector surface may dissolve into the liquid, causing absorption of scintillation light and degradation of detector performance. Among these impurities, water is the one most likely to affect the propagation of liquid xenon scintillation as its absorption cross section overlaps with the xenon scintillation light spectrum. In order to efficiently remove the water dissolved into the liquid, the xenon is circulated in the liquid phase by a low-temperature liquid pump through a filter containing molecular sieves with a pore size 13A, which is suitable to remove water molecules. In the MEG experiment, 70L/hour circulation is achieved with this system, resulting in preparing sufficiently pure liquid in a reasonable time.

\textbf{4. Small refrigerator}:
As used in the MEG experiment, a small refrigerator installed on the top the detector is used to liquefy xenon and re-liquefy the constantly evaporating xenon gas. The use of a pulse-tube refrigerator is suitable from the viewpoint of low vibration noise, but to obtain a high refrigeration power, a GM-type refrigerator can be installed at a distance from the detector with a vacuum insulated pipe to transfer the liquid to the detector. Both types of refrigerators have been used in MEG, and there are no technical difficulties.

\textbf{5. Temperature and pressure control system}:
The cryostat is always subject to heat by conduction through the support structure and cables as well as heat generation from electronics circuits and photo sensors placed in the cryostat. After liquefaction completes, the liquid xenon evaporates continuously due to the heat generated by these, and the pressure rises. In order to control the temperature and pressure of the liquid xenon, xenon is re-liquefied by the refrigerator. In order to maintain the liquid state at a temperature and pressure suitable for operation, the refrigerator cooling power is controlled by changing the heater output on the cold head while the refrigerator continues to operate at maximum capacity. This method has already been used in MEG and many other experiments using liquid xenon, and there is no problem in maintaining the stability of the liquid.
%\el

==> PioneerExperiment/Trigger/electronics.tex <==


\subsubsection{Trigger design}
\label{Trigger}
Figure~\ref{fig:readout} shows the planned topology for readout and triggering of PIONEER.  The design takes advantage of
the APOLLO~\cite{ApolloTWEPP21} platform designed for the trigger track finder and pixel readout in the CMS experiment at
the LHC.  The Command Module (CM) component of the APOLLO board provides a highly configurable environment supporting a dense
high speed IO environment via
%104 16 to or 
25 Gbps Samtec Firefly~\cite{firefly} optical inputs.  The platform already
supports the flexible high speed synchronous command and triggering TCDS2 (Trigger and Timing Control and Distribution
System)~\cite{CMSP2TDR} for the CMS phase II upgrade, as well as options for direct IO for receiving timing signals or
generating trigger signals for devices expecting analog triggers.  We anticipate using a single FPGA version of the board (utilizing the Xilinx VU13P) with an interposer in the second FPGA slot to bring all the serial links to the VU13P.
While by some measures this board likely provides more power than needed for PIONEER, it has already undergone significant prototyping with full production anticipated in 2024, and can satisfy several of the needs of the system with a single platform.  The engineering group that designed the CM will also contribute to calorimetry readout, providing additional coherence.  

\begin{figure}[tb]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/TriggerBackend.pdf}
\caption{Proposed topology of the trigger and subdetector readout systems.}
\label{fig:readout}
\end{center}
\end{figure}

PIONEER anticipates use of the 16.1 Gbps Firefly implementation. This protocol serializes 64 bit words with a 64b/66b encoding, resulting in an effective transmission of 64 bit words at rates up to 244\,MHz.  Each channel supports both transmit and receive functions, which will allow for significant flexibility in the command and control system.

The Samtec Firefly system already supports PCI Express (PCIe) Gen 3 and Gen 4 integration, with commercial PCIe over firefly adapter cards already available for Gen 3.  As discussed further in Sec.~\ref{subsec:daq}, PIONEER proposes use of PCIe as the protocol underlying the DAQ system.

The main trigger APOLLO processor will receive trigger inputs, either via inputs connected to the FPGA standard IO pins, or from the firefly inputs and apply the appropriate logic algorithms to generate triggers and guide sparsification.  The processors  encode the resulting trigger and configuration information into the TCDS (or equivalent) datastream, which gets transmitted to all subdetectors.  The processor will also receive status and health information from the subdectector, communicating any alarm conditions to the DAQ system for appropriate action.  

The trigger processor will receive trigger inputs from the BEAM counters and from the tracker to form the PI, Track and PROMPT triggers, with configurable prescale factors applied as noted earlier.  The processor will also receive energy sums from subsections of the calorimeter (see Sec.~\ref{subsec:caloBE}) and complete the total energy sum used to form the CaloH trigger in coincidence with the (unprescaled) PI trigger.  The processor can flexibly accommodate the needs of the beta decay (Phase II) of the experiment, completing, for example, opening angle or mass estimates based on energy-weighted position sums from the calorimeter electronics.

The processor will also interact with the ATAR, level 3 trigger system and DAQ system to coordinate additional trigger information from the patterns in the ATAR as described above.

\subsubsection{Calorimeter backend electronics}
\label{subsec:caloBE}
Figure~\ref{fig:calodaq} illustrates the digitization and readout electronics proposed for the calorimeter.  The 12 channel digitization boards will utilize the Analog Devices AD 9234 dual channel, 12 bit 1 GSPS ADC chip, chosen for its low latency of 59\,ns from presentation of the signal at the front end to output of the digitized signal.  These chips communicate the digitized output via the JESD204 protocol, which will present the data for each ADC channel as 64 bit words containing four samples at 250\,MHz.  At these rates, the calorimeter information can be summed with a pipelined adder and potentially corrected with a running pedestal measurement as the first stage in a total energy measurement.  By clocking the ADC at the slightly lower rate of 976\,MHz, the ADC information can be synchronized to the firefly data transfer rate of 244\,MHz, simplifying synchronization of the system.

The ADCs will sample continuously with samples stored initially in a ring buffer on the FPGA.  Upon receipt of a trigger, a configurable time window will be stored in DIMM memory.  By deploying a DIMM with a 128 bit data path, simultaneous reading and writing can be accomplished via two 64 bit pathways.

\begin{figure}[tb]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/CaloDAQ.pdf}
\caption{Proposed calorimeter digitization and readout.  The 12 channel digitizer boards utlize the dual channel AD9234 12 bit, 1 GSPS ADCs, Xilinx Ultrascale FPGAs for contro, and Samtec Firefly\textsuperscript{TM} high speed communications to a CMS APOLLO board.  The APOLLO board can receive up to 22 boards in this configuration -- instrumenting quadrant of an order 1000 channel calorimeter.}
\label{fig:calodaq}
\end{center}
\end{figure}

A single FPGA will control one pair of ADCs (four calorimeter channels).  It can compare the energy sum from each channel against a channel activity threshold (or thresholds), as well as combine the four running energy sums as the first stage of a total energy sum for the high energy trigger.  That FPGA will also drive a single firefly channel.  The 64 bit word for the firefly communication provides much flexibility.  After reserving 48 bits for readout of the four channels upon receipt of a trigger, 16 bits can provide triggering information at the full 244\,MHz rate.  Possible configurations include a 12 bit sum of the four calorimeter channels along with a bit for each channel flagging a sum over threshold.  With a coarse 8 bit sum, 2 bits could be devoted to each individual channel.  For the beta decay phase, the trigger could pass energy-weighted position information for a mass calculation. Xilinx kintex ultrascale FPGAs provide sufficient numbers of high speed serial lines at a reasonable cost.

The digitizer boards will communicate with intermediate Apollo boards via the 16.1\,GHz firefly links, which come packaged with a minimum of four individual links.  Three of these links will provide the TCDS (or equivalent) clock and control signals and send the trigger and channel readout information to each of three sets of 4 ADC channels.  The fourth firefly line will provide PCIe or ethernet communication to allow board configuration and other slow control functions.

After taking into account communication links to the trigger processor and between the intermediate Apollo boards, each intermediate Apollo can accommodate 22 12-channel digitizer boards for a total of 264 channels. Four such boards would instrument a calorimeter with up to 1056 channels.  With a more complex, run-state dependent scheme for communications, 16 channels per board could be accommodated.

The intermediate APOLLO boards will collate the waveforms read from all channels for each trigger, and send that information directly to the DAQ system.  Each APOLLO can sustain a full readout rate of about 18.5 kHz for the 264 channels, allowing for significant headroom given the anticipated trigger rates (see Tab.~\ref{tab:triggers}) and use of sparsification for an order 1000 channel calorimeter.

The total calorimeter energy sum proceeds in several stages.  Each quad-channel FPGA adds those four signals as noted above.  Each intermediate Apollo will combine the those sums from the $22\times 3=66$ quad channels.  The trigger process will provide the final combination of the four intermediate sums needed for the complete calorimeter sum. 

The latency in the energy sum has three main contributions: the ADC latency, the FPGA summation time, and the serialization/deserialization overhead for the high speed links.  The Xilinx GTY transceivers have a high degree of configurability, resulting in a total serialize/deserialize latency for the readout chain above that ranges from 65\,ns to 175\,ns at the 16.1\,GHz serial rate.  Recent studies~\cite{OliveiraThesis} show that even the simpler, lower latency settings, can achieve reliable links.  With 100~ns as a reasonable estimate, 50\,ns as a limit for the energy summation at 244\,MHz, and the 50\,ns ADC latency, we estimate a total latency of 200\,ns.

==> PioneerExperiment/Trigger/trigger.tex <==
All triggers will start with a PI signal, which is a loose condition for an incident beam particle. PI can be defined as a coincidence
of the BEAM detectors (LGAD telescope layers). The key point is that this trigger must not introduce any bias between \pie\ and \pme\ events. For the estimates we assume that a separator is installed, so that the rate R$_{PI}$=300\,kHz corresponds to the design beam rate and is dominated by pions.

The main time distributions in the vicinity of the PI signal are sketched in Fig.~\ref{fig:time}. After an initial build-up with the pion lifetime,  positron rates from \pme\ reach their maximum before decreasing with the muon lifetime. The constant accidental rate from muon decays of other pions stopped in ATAR is high.

\begin{figure}[htb]
\centering
\includegraphics[width=0.7\textwidth]{Figures/Trigger/times.png}
\caption{Positron rates after PI per second in 1\,ns time bins. \pie\ positron rates are multiplied by a factor 100.  \pme\ rates generated by PI shown in red and positron rates from old muons, i.e. from accidental pions, shown in blue. }
\label{fig:time}
\end{figure}

After requiring the PI signal, the following main triggers are formed:
 \bl [enumerate]
\ListProperties(Start1=1)
& \tpi: This is a minimum bias trigger, with the PI signal prescaled by about k=1000.
& \tcaloh: Selection of high energy (E$_{tot} \gtrsim$ \thcal) events detected by the \calo\ within a time range TR=[-300,700] ns relative to PI.
& \ttrack: All events with \track\ hit within time range TR relative to PI, prescaled by about k=50. We note that the probability to observe a \pme\ positron in TR is 0.19, while the probably for detecting an old muon positron is 0.3, thus accidentals are a significant part of this trigger.
& \tprompt: Selected prompt events with a \track\ hit in time range [2,32] ns relative to PI, potentially prescaling required.
\el





For all triggers a full event readout will be initiated. 
The properties and required bandwidth for these trigger classes are summarized in Table~\ref{tab:triggers}. Additional data flow from the \track\ and \beam\ counters is small, and not included.

\begin{table}[htbp]
  \centering
  \small
    \begin{tabular}{cccc|ccc|ccc|cc}
    \toprule
    triggers & prescale &  range & rate & \multicolumn{3}{c|}{\calo} & \multicolumn{3}{c|}{\atar\ digitizer} & \multicolumn{2}{c}{\atar\ high thres} \\
          &       &  TR(ns)     &   (kHz)     & $\Delta$T(ns) & chan  & MB/s  &$\Delta$T(ns) & chan  & MB/s  & chan  & MB/s \\
       \hline
    \tpi  		& 1000  & -300,700 	& 0.3   & 200  	& 1000 	& 120 	& 30    & 66    & 2.4 & 20    & 0.012 \\
    \tcaloh 	& 1     & -300,700 	& 0.1  	& 200 	& 1000 	& 40 	& 30    & 66    & 0.8 & 20    & 0.004 \\
    \ttrack 	& 50  	& -300,700 	& 3.4  	& 200  	& 1000 	& 1360  & 30 	& 66    & 27 & 20    & 0.014 \\
    \tprompt 	& 1     & 2,32  	& 5     & 200  	& 1000 	& 2000 	& 30    & 66    & 40  & 20    & 0.2 \\
    \bottomrule
    \end{tabular}%
  \caption{Main triggers: time range TR and  trigger rates. For detector systems readout island length $\Delta$T, average number of channels and required readout bandwidth are given.  }
  \label{tab:triggers}%
\end{table}%

The main purpose of \tcaloh\ and \ttrack\ is the selection of true \pie\ and \pme\ events, respectively. The $E_{tot}$ \calo\ energy sum will be calculated in the trigger processor with a latency of 200\,ns. Events above the Michel continuum with $E_{tot} >E_H \approx$ \thcal\ will be assigned to \tcaloh.

The full event readout includes the \calo\ waveforms, the \atar\ and the \beam\ and \track\ detectors.

The \calo\ data  will comprise islands of contiguously digitized ADC samples from the SiPMs / PMTs readout of the calorimeter. We assume 2-bytes per sample, 200 samples per island, and 1000 islands channels per trigger. Thus a trigger rate of 5\,kHz generates 2\,GB/s.

The zero suppressed \atar\ waveforms of typical length of $\Delta$T=30 ns will be stored,  
with the readout window extended if the signal remains above threshold at the end of the island.
The dominant \pme\ event will fire about 66 strips. Depending on strip cross talk, which differs for LGAD technology choices, i.e. AC-LGAD vs. TI-LGADS, this strip count could be 3-times higher.  With a 1 GSa/s digitization and 4 Bytes required per hit, 66 channels of 30 ns islands correspond to 30*66*4=8 kB. Thus a trigger rate of 5\,kHz generates 40 MB/s.

In addition (see \atar\ high thres in Table~\ref{tab:triggers}) the trigger processor will also receive high threshold logic signals from the \atar\ low and high threshold discriminators located at the frontend of the ATAR digitizers and will time stamp those with coarse resolution (few ns). Those hits will always be read out for a time period of 10\,$\mu$s preceding PI. This data can determine whether  a previous pion stopped at the stop location of PI, to potentially apply a local pile-up for those events. 

By far the most challenging is the \tprompt\ trigger which is of critical importance for the experiment. 
\bl
\ListProperties(Margin=2cm, Hang1=true,Hide2=0,Numbers1=r,Numbers2=r,Progressive*=.5 cm,Start1=1)
& It will trigger on all prompt \ttrack\ events, where the \pme\ events are suppressed by a factor 6.4$\times 10^{-3}$ in [2,32] ns. This should verify that the \tcaloh\ trigger does not miss events by its more complicated E$_{tot}$ trigger configuration. If required this part of the trigger can be prescaled.
& \tprompt\ is critical to measure \pie\ events which are lost because the CALO response falls below $E_H$. The uncertainty in those losses were the limiting systematics in the last generation of experiments. We consider additional \atar\ requirements at trigger level, like hits in the most upstream layers and no hit in the most down stream layers within the \atar\ time resolution of 100\,ps. We will design the trigger processor and DAQ bandwidth such that all \tprompt\ events can be transferred in streaming mode to a front end computer farm. Thus the stored data volume will be reduced in a combination of trigger processor and software decisions, by applying \atar\ cuts on track topology and energies to suppress \pme\ events. 
Ideally, this should be done in an unbiased way. However, as the main purpose
is a measurement of the loss term of \pie\ events, small biases can be tolerated and even prescaling can be considered if unavoidable.

&
In addition, the \tprompt\ trigger will select a sample of \pdar-\mdif\ events. Positrons from immediate \mdif\ decay are indistinguishable from the
\pie\ radiative tail events. Measurements of the spectrum of positrons after PI, where the muon deposits only a fraction
of its 4\,MeV energy, will constrain this background class.
\el
 

==> Planning/Cost.tex <==






%Table~\ref{cost} indicates the estimated costs of the PIONEER experiment assuming that the MEG 1000~l LXe supply (estimated value CHF 7.5M) will be used. 

\begin{table}[htbp]
    \centering
    \begin{tabular}{p{3in}r}
    \toprule
    PIONEEER Cost Estimate & M ChF \\
    \hline
    R\&D & 2.0 \\
    ATAR & 1.3 \\
    Trackers/Beam instr. & 0.5 \\
    Calorimeter & 20.3 \\
    Trigger/DAQ & 1.0 \\
    Other & 1.0 \\
    {\bf Total} & {\bf 26.1} \\

    \bottomrule
    \end{tabular}
\caption{ PIONEER preliminary cost estimate, assuming that the MEG 1000~l LXe supply (estimated value CHF 7.5M) will be used.}
\label{tab:cost}
\end{table}

%\begin{figure}[htbp]

%\centering
%\includegraphics[scale=0.5]{Figures/CostEstimate.pdf}
%\caption{ PIONEER preliminary cost estimate.}
%\label{cost}
%\end{figure}

==> Planning/alphCollaboration.tex <==
\author{W.~Altmannshofer}\affiliation {University of California Santa Cruz}
\author{H.~Binney}\affiliation{University of Washington}
\author{E.~Blucher}\affiliation{University of Chicago}
\author{D.~Bryman}\affiliation{University of British Columbia}\affiliation{TRIUMF}
\author{S.~Chen}\affiliation { Tsinghua University  }
\author{V.~Cirigliano}\affiliation{Theoretical Division, Los Alamos National Laboratory}%, Los Alamos, NM 87545, USA}
\author{S.~Corrodi}\affiliation{Argonne National Laboratory}
\author{A. Crivellin}\affiliation{Paul Scherrer Institute}\affiliation{University of Zurich}\affiliation{CERN}
\author{S.~Cuen-Rochin}\affiliation{Tec de Monterrey}
\author{A.~Di Canto}\affiliation{Brookhaven National Laboratory}
\author{L.~Doria}\affiliation{Johannes Gutenberg University Mainz}
\author{A.~Gaponenko}\affiliation{Fermilab}
\author{A.~Garcia}\affiliation{University of Washington}
\author{L.~Gibbons}\affiliation{Cornell University}
\author{C.~Glaser}\affiliation {University of Virginia}
\author{M.~Escobar~Godoy}\affiliation {University of California Santa Cruz}
\author{D.~G\"oldi}\affiliation{ETH Zurich}
\author{S.~Gori}\affiliation {University of California Santa Cruz}
\author{T.~Gorringe}\affiliation{University of Kentucky}
\author{D.~Hertzog}\affiliation{University of Washington}
\author{Z.~Hodge}\affiliation{University of Washington}
\author{M.~Hoferichter}\affiliation{University of Bern}
\author{S.~Ito}\affiliation{KEK}
\author{T.~Iwamoto}\affiliation{University of Tokyo}
\author{P.~Kammel}\affiliation{University of Washington}
\author{B.~Kiburg}\affiliation{Fermilab}
\author{K.~Labe}\affiliation{Cornell University}
\author{J.~LaBounty}\affiliation{University of Washington}
\author{U.~Langenegger}\affiliation{Paul Scherrer Institute}
\author{C.~Malbrunot}\affiliation{TRIUMF}
%\author{W. Marciano}\affiliation{Brookhaven National Laboratory}
\author{S.M.~Mazza}\affiliation {University of California Santa Cruz}
\author{S.~Mihara}\affiliation{KEK}
\author{R.~Mischke}\affiliation{TRIUMF}
\author{T.~Mori}\affiliation{University of Tokyo}
\author{J.~Mott}\affiliation{Fermilab}
\author{T.~Numao}\affiliation{TRIUMF}
\author{W.~Ootani}\affiliation{University of Tokyo}
\author{J.~Ott}\affiliation {University of California Santa Cruz}
\author{K.~Pachal}\affiliation{TRIUMF}
\author{C.~Polly}\affiliation{Fermilab}
\author{D.~Po\v{c}ani\'c}\affiliation {University of Virginia}
\author{X.~Qian}\affiliation{Brookhaven National Laboratory}
\author{D.~Ries}\affiliation{Johannes Gutenberg University Mainz}
\author{R.~Roehnelt}\affiliation{University of Washington}
\author{B.~Schumm}\affiliation {University of California Santa Cruz}
\author{P.~Schwendimann}\affiliation{University of Washington}
\author{A.~Seiden}\affiliation {University of California Santa Cruz}
\author{A.~Sher}\affiliation{TRIUMF}
\author{R.~Shrock}\affiliation {Stony Brook University}
\author{A.~Soter}\affiliation{ETH Zurich}
\author{T.~Sullivan}\affiliation{University of Victoria}
\author{M.~Tarka}\affiliation {University of California Santa Cruz}
\author{V.~Tischenko}\affiliation{Brookhaven National Laboratory}
\author{A.~Tricoli}\affiliation{Brookhaven National Laboratory}
\author{B.~Velghe}\affiliation{TRIUMF}

\author{V.~Wong}\affiliation{TRIUMF}
\author{E.~Worcester}\affiliation{Brookhaven National Laboratory}
\author{M.~Worcester}\affiliation{Brookhaven National Laboratory}
\author{C.~Zhang}\affiliation{Brookhaven National Laboratory}
% OPT out
%\author {A. Knecht}%\affiliation{PSI}
%\author {D. Salvat}%\affiliation{Indiana University}
%\author{A.~Czarnecki}\affiliation{University of Alberta}
%\author{D.~Jaffe}\affiliation{Brookhaven National Laboratory}
%\author{S.~Kettel}\affiliation{Brookhaven National Laboratory}
% No response
%\author{T.~Wataru}\affiliation{University of Tokyo}
%\author{A.~Grillo}\affiliation {University of California Santa Cruz}
%\author{M.~Gorchteyn}\affiliation{Johannes Gutenberg University Mainz}
%\author{C.~Ortega Hernandez}\affiliation{Universidad Nacional Autonoma de Mexico}

==> Planning/collaboration.tex <==








\author {W. Altmannshofer, S. Gori, M. Godoy, A. Grillo, S. Mazza, J. Ott,  B. Schumm, A. Seiden, M. Tarka}
\affiliation {University of California Santa Cruz}
\author {H. Binney, A. Garcia, D. Hertzog, Z. Hodge, P. Kammel, J. LaBounty, R. Roehnelt}
\affiliation { University of Washington  }
\author {E. Blucher}
\affiliation{University of Chicago}
\author {D. Bryman}
\affiliation{University of British Columbia  and TRIUMF}
\author {S. Chen}
\affiliation { Tsinghua University  }
\author {V. Cirigliano}
\affiliation{ Los Alamos National Laboratory}%, Los Alamos, NM 87545, USA}
%\author {A. Crivellin}
%\affiliation{Paul Scherrer Institute, University of Zurich}

\author{S. Corrodi}
\affiliation{Argonne National Laboratory}

\author { C. Ortega Hernandez}
\affiliation{Universidad Nacional Autonoma de Mexico}
\author{S. Cuen-Rochin}
\affiliation{Tec de Monterrey}
\author {A. Czarnecki}
\affiliation{University of Alberta}
\author {A. DiCanto, D. Jaffe, S. Kettel,
%W. Marciano, 
V. Tischenko, A. Tricoli, E. Worcester}
\affiliation {Brookhaven National Laborory}
\author {L. Doria, M. Gorchtein, D. Ries}
\affiliation{ Johannes Gutenberg University Mainz}
\author {A. Gaponenko, B. Kiburg,J. Mott, C. Polly}
\affiliation {Fermilab}
\author {L. Gibbons, K. Labe}
\affiliation{Cornell University}
\author {C. Glaser, D. Po\v{c}ani\'c}
\affiliation {University of Virginia}
\author {T. Gorringe}
\affiliation{University of Kentucky}
\author { M. Hoferichter}
\affiliation { University of Bern  }
\author{S.  Ito, S. Mihara}
\affiliation {KEK}
\author {T. Iwamoto, T. Mori, W. Ootani, T. Wataru}
\affiliation {University of Tokyo  }
%\author {A. Knecht, U. Langenegger}
\author {P. Schwendimann, U. Langenegger}
\affiliation{PSI}
\author{ C. Malbrunot}
\affiliation{CERN}
\author { R. Mischke, T. Numao, K. Pachal, A. Sher, B. Velghe, V. Wong}
\affiliation{TRIUMF}
%\author { D. Salvat}
%\affiliation{Indiana University}
\author  {A. Soter}
\affiliation{ETH Zurich}
\author  {R. Shrock}
\affiliation {Stony Brook University}
\author {T. Sullivan}
\affiliation{University of Victoria}


==> SimAnal.tex <==
\subsection {Beam and beam instrumentation}
\subsection {LXe Calorimeter}
\subsection {ATAR}


==> Simulations and Analysis/Geant4simulations.tex <==






\section{Simulations} \label{Sims}





Each of the design elements discussed above is being actively studied %and iterated upon 
using GEANT4-based \cite{GEANT4:2002zbu} simulations.
%to study the performance of each element in detail. 
The simulation efforts include 
%breaks down nicely into 3 parts: 
beamline and upstream detector simulations, simulation of the active target, and simulation of the calorimeter. 

The $\pi$E5 beamline at PSI is simulated using G4Beamline \cite{Roberts:2008zzc} discussed in Section \ref{sec:beam_studies}. The remainder of the simulation is done primarily using GEARS, %\cite{gears}, 
an extension of GEANT4, which streamlines readout for rapidly iterating systems. The geometries for each of the experimental components are generated using a stand-alone Python script and geometry library, which takes as its input a \texttt{json} file of various parameters (e.g. diameters, number of elements, which detectors to implement, etc.) and exports a \texttt{GDML} file which is then read in by the Geant4 simulation. This file contains a full description of the physical geometry of the detectors, as well as their material properties (density, reflectivity, scintillation yield, etc.). 
Because of this workflow, it becomes trivial to implement scans over various parameters to perform systematic studies. 

%TODO: Tools paragraph (geant4, g4beamline, trim, ...)

In the following sections, we discuss the initial ATAR and calorimeter simulations.



\subsection{ATAR Simulations}

Simulations of the active target are done with both GEANT4, which allows us to model pions and their decay products through the full chain of detectors, and 
TRIM\cite{ziegler1985stopping}, 
which allows us to track particle energy deposition precisely in a simulated detector readout. 
Figure \ref{fig:atar_sim} (left) shows the ATAR concept  and (right) a simulation of energy deposit by exiting positrons as a function of polar angle of emission.
\begin{figure}
   \centering
   \includegraphics[width=0.35\textwidth]{Figures/Simulation/atar_image.png}
   \includegraphics[width=0.48\textwidth]{Figures/Simulation/atar_deposited_energy.pdf}
   \caption{Left: An image of the simulated ATAR, showing the active planes (white) and readout strips (orange). Right: Total energy deposited in the ATAR by the decay positron as a function of the angle $\theta$ at which it enters the calorimeter. }
  \label{fig:atar_sim}
\end{figure}

The active target is implemented in the simulation as alternating layers of cross-hatched silicon strips. The number of strips per layer, their thicknesses, and the number of layers is fully configurable. The nominal configuration consists of 48 \unit[120]{$\mu$m} thick planes of 100 strips each for a total size of $\unit[20 \times 20 \times 5.76]{mm^3}$. Optional `dead' zones can be implemented in each pixel, to simulate the effect of trenches between pixels within a plane or a dead backing layer. Each plane of the ATAR has a fully simulated readout cable, consisting of Kapton and Silicon,  simulating the ultimate flex cable readout. These readouts introduce an asymmetry in the energy reconstructed by the calorimeter, and as such have the potential to introduce a systematic bias to our analysis. The design of the readouts will be informed by this simulation in order to minimize such an effect.

\subsubsection{ Background  Suppression for the Measurement of the \pie\ tail fraction}
%\label{tail_suppression}
\input{Simulations and Analysis/SuppressedBackground}

There is an ongoing effort to apply machine learning tools to boost the sensitivity to $\pi^{+}\rightarrow e^{+}\nu$ events in the tail region and suppress the backgrounds. It has already been demonstrated with the in-ATAR $\pi\,\mathrm{DIF}$ events that gradient boosting decision trees (BDT) are able to  outperform the manual cut-based methods.  %Details of the BDT study can be found in Appendix ~\ref{sec:DIFsuppression_BDT_appendix}.
Although the BDT model shows excellent classification performance, only manually-constructed physics-inspired high-level information has been used as input features for the model training. As deep neural networks, especially Convolutional Neural Networks (CNN), have shown extraordinary performance in various image processing and classification applications, it could be advantageous to make use of deep neural networks’ ability to automatically learn high-level features directly from the complete pixel-level energy deposit information.
%Figure ? shows the idea of a composite algorithm consisting of a BDT that learn on high-level feaures and a CNN that learn on low-level ATAR energy deposit images, whose outputs are then combined in a final neural network layer. 

\subsection{Calorimeter Simulations}
\label{sec:calo_simu}

%\begin{itemize}
   % \item Perform tail calculation for various nX0; 
 %   \item Show feasibility of handling pile up for \pie~ and pion beta decay (LXe)
   % \item Examine feasibility vs energy resolution for pi->enu, pion beta decay (LYSO)
   % \item Examine hybrid configurations: PiBeta CSI+LYSO; PiBeta CSI+ tail catcher veto
%\end{itemize}

%\subsubsection{LXe Calorimeter Design}

% We use GEANT4-based \cite{GEANT4:2002zbu} simulations to study the performance of the LXe calorimeter, in particular, with respect to photo-nuclear interactions, the low energy tail determination and pile-up rejection.

\subsubsection{Pileup}

Simulation studies of the LXe calorimeter response have been performed using the GEANT4 package \cite{GEANT4:2002zbu} with optical photon tracking. A simple geometry (see Fig.~\ref{fig:geometry_MC}) that is representative of the current design was implemented. $\pi\rightarrow \mu\rightarrow e$ events were generated in the target at the center of the LXe sphere and optical photons originating from LXe scintillation induced by the showers generated by the positrons were tracked until the outside sensitive surface of the LXe sphere. The  simulated 
pulses obtained are similar to the ones reported by  MEG.
A pulse fitting algorithm was employed to evaluate the possibility of separating events that overlap in time i.e.~pulse  pileup. Pulse separation down to \unit[5]{ns} was achieved (see illustration in Fig.~\ref{fig:PSF}) across a wide range of amplitudes. This gives a first indication (without digitization) of the performance of the detector and subsequent data analysis with respect to dealing with  pileup.

Further studies are anticipated to introduce and optimize optical qualities of the surfaces, optimize photo-sensing detectors' coverage,
and improve the simulation of the originating scintillation photons. Much  of the input for these simulations will be  provided by test measurements. 
\begin{figure}[!tbp]
  \centering
  \subfloat[]{\includegraphics[width=0.22\textwidth]{
  Figures/geometry_MC.pdf}\label{fig:geometry_MC}}
  \hfill
%   \subfloat[]{\includegraphics[width=0.7\textwidth]{Figures/PSF_new.pdf}\label{fig:PSF}}
  \subfloat[]{\includegraphics[width=0.7\textwidth]{Figures/Simulation/lxe_pulse_fit_updated.pdf}\label{fig:PSF}}
  \caption{(a) Rendering of the simplified geometry used in the first Monte-Carlo simulation of the PIONEER LXe calorimeter (b) Example of simulated pulse shapes of a single $\pi\rightarrow \mu \rightarrow e$ event (top) and 3 events happening closely in time (bottom) and recorded in the LXe calorimeter. Pulse shape fitting based on a template allows accurate identification and energy reconstruction of multiple pulses down to $\pm$\unit[5]{ns} separation.} % add some caveat
\end{figure}
Position resolution will  also augment  pile-up handling capabilities. The position resolution capabilities of the detector and its importance for achieving the targeted rate will be modeled  and studies  are envisaged in the apparatus which will also be used to test the photo-sensors in LXe.  
Depending on the outcome of the pileup studies, segmentation of the LXe volume may be considered.
%although there are complicating factors due to the UV scintillation light. 
 



\subsubsection{Additional Calorimeter Studies}

At the current design stage and given the targeted level of precision, further simulations assessing the performance of the calorimeter will be carried out in conjunction with development of design parameters for the beam, ATAR, and  tracking detectors. 
%Simulation data that is being analyzed by collaborators from several institutions.
One important aspect of the calorimeter design that is being informed by the simulations is understanding how energy from a decay positron is `lost' before it reaches the calorimeter. While energy lost in the ATAR is measured,  losses occurring in inactive material  e.g. the ATAR cabling, and calorimeter entrance windows, depend on the angle of emission.    Simulations are being used to study these effects on the positron energy  resolution.  


Another important study involves modeling of photonuclear interactions. As decay positrons interact with atomic nuclei in the simulation, they will occasionally cause a nucleus to enter into an excited state with single or multiple neutron emission. When these neutrons escape the calorimeter without depositing their energy the observed energy is shifted down by multiples of the neutron binding energy (see Fig.~\ref{fig:Signal-Tail}). Photonuclear processes were studied in the PIENU experiment to determine the impact on the NaI(Tl) calorimeter lineshape.  The results were used as input to the calorimeter simulations. Modeling and prototype studies will be pursued for evaluating these effects in LXe. 

% This is speculation which hasn't been studied:
%Photonuclear interactions can also contribute to pileup. The energy from a single positron can create multiple light peaks in the detector. This can be caused by a neutron ejected from a nucleus travelling some distance within the calorimeter before being reabsorbed or a nucleus which has been excited that decays at some later time. Information from the ATAR and tracker can be used to identify and study these events by selecting isolated, single positron tracks.



In summary, the robustness of the calorimeter performance for the determination of the low energy tail, the resolution,  and the pileup rejection will be evaluated by studying  the following aspects:

\begin{itemize}
    \item impact on resolution and reconstruction of energy loss in inactive materials,
    \item optical properties of the inner surfaces of the LXe detector (reflectivity, light absorption, etc),
    \item granularity, layout (inner and outer surfaces) and specification of photo-sensors (dark current, PDE, etc.), and
    \item characterizations of scintillation light in LXe;  e.g., variations in the absorption length.
\end{itemize} 
Understanding how these conditions affect the performance of the calorimeter will determine the critical parameters required for the next phase of the experimental design.

==> Simulations and Analysis/Suppress0.tex <==








With an anticipated tail fraction of f=0.5\% of \pie~ events, $\mu-e$ decays must be suppressed to a level that allows measurement of f with accuracy 1-2\%. This can be accomplished by using ATAR information to identify stopped pions by energy loss, and range-energy relations, using a narrow time window (e.g. 3-35 ns) following the pion stop, observing the 4.2 MeV decay muon, and suppressing events with pion DIF, and muon DIF following pion DAR by tracking and energy loss measurements.

%Suppressing events mimicing $\pi^{+}\rightarrow e^{+}\nu$ decays from  decay-in-flight $\pi^{+} \rightarrow \mu^{+} \nu$ events in the “low energy tail” region. 
As illustrated in Figure \ref{fig:EventTypes}, a background source of $\pi^{+} \rightarrow \mu^{+} \rightarrow  e^{+}$ events comes from pions that decay in flight ($\pi\,\mathrm{DIF}$) either in the ATAR or upstream, followed by muon  decay at rest. 
In addition,  muons that originate from pion DAR in the ATAR can decay in flight before stopping ($\mu\,\mathrm{DIF}$), leaving a positron with the same time distribution as the ones in a $\pi^{+}\rightarrow e^{+}\nu$ events. 
%Table ? indicates the proportions of each types of decay-in-flight events to the decay-at-rest $\pi^{+}\rightarrow e^{+}\nu$ events.
With high granularity and sub-ns timing resolution, the ATAR  can observe the energy deposits of the pion decay products, and thus identifying these different decay modes.
Figure ? shows the distribution of the $\pi$ decay vertex position along the beam direction for the various decay modes of $\pi^{+} \rightarrow \mu^{+} \nu$ events. The individual ATAR event display of some $\pi^{+}\rightarrow e^{+}\nu$ and $\pi^{+} \rightarrow \mu^{+} \rightarrow  e^{+}$ examples are included in Appendix ?. 

Initial studies indicate that the $\pi\,\mathrm{DIF}$ events can be rejected by a suppression factor of 50 using an early decay positron timing window of 5-35 ns (see Figure ?). 
It has been studied with the simulation that the in-ATAR $\pi\,\mathrm{DIF}$ events can be further reduced by a suppression factor of 200 with a traditional cut-based method when the ATAR information is utilized to determine the pion decay position, the existence of kinks in the topology, and dE/dx along the track. 
Under the conservative assumption that 1\% of $\pi^{+}\rightarrow e^{+}\nu$ events would lie in the tail region, this results in an estimation of 0.09 in-ATAR $\pi\,\mathrm{DIF}$ event per $\pi^{+}\rightarrow e^{+}\nu$ event. 
To mitigate the events where the pion decay-in-flight between the degrader and the ATAR, an upstream tracker will be placed right in front of the degrader to provide the tracking of the incoming pion. If the pion decay in flight between the degrader and the ATAR, a non-zero kink angle between the track in the upstream tracker and the one in the ATAR will be detected. This would highly suppress the upstream $\pi\,\mathrm{DIF}$ events.

For the $\mu\,\mathrm{DIF}$ event, although the probability of occurrence is much smaller, it had been a dominating source of tail corrections in previous experiment, as it has the same decay positron time distribution. Thanks to the high granularity of the ATAR, it is possible to set apart the energy deposition of the closely-happening muon and positron, or even measure their energy loss along the decay length. It is expected that a muon decays in roughly 1 mm, and thus leaving hits in 4 strips on average. From a simulation of $\mu\,\mathrm{DIF}$ events, a suppression factor of 18 was recognized with the separation power from dE/dx measurement. This leads to 0.08 $\mu\,\mathrm{DIF}$ events per $\pi^{+}\rightarrow e^{+}\nu$ event. As a whole, the simulation studies indicate that all the $\mathrm{DIF}$ background events together could be suppressed to a level of 10\% or smaller, allowing the experiment to achieve a tail correction uncertainty as low as 1\%.

\begin{itemize}
  \item For upstream $\pi\,\mathrm{DIF}$ event, hopefully we will have some numbers to update. Otherwise, maybe we can try to quote a conservative number from PIENU’s experience. 
  \item For $\mu\,\mathrm{DIF}$ event, we might update some numbers after seeing how kink topology might help as well.
\end{itemize}



==> Simulations and Analysis/SuppressedBackground.tex <==



\label{tail_suppression}

With an anticipated tail fraction $f= 0.5\%$ of \pie\ events, $\mu-e$ decays must be suppressed to a level that allows measurement of $\Delta f/f$  with accuracy 1--2\%. This can be accomplished by using ATAR information to identify stopped pions (and reject incoming muons) by energy loss, and range-energy relations, using a narrow time window (e.g. 3--35\,ns) following the pion stop, rejecting events with observation of the \tmu\ decay muon, and suppressing events with pion decay-in-flight (\pdif), and muon decay-in-flight (\mdif) following pion decay-at-rest (\pdar) by tracking and energy loss measurements. 
%Special background-suppressed runs will be taken to determine $f$.

Assuming a 10\% energy resolution (comparable to that of the PIENU target) $\pi\to\mu\to e$ background in the tail region from the dominant pion decay at rest will be suppressed to a negligible level as found in PIENU. Radiative decays $\pi\to\mu \nu \gamma$ followed by $\mu\to e$ decays which may leave $<4.1$ MeV in the target will be suppressed by observation of the gamma and  detection of the muon pulse and residual energy. In addition, muons that originate from \pdar\ in the ATAR can decay in flight in the 12\,ps it takes  before stopping ($\mu\,\mathrm{DIF}$), leaving a positron with the same time distribution as $\pi^{+}\rightarrow e^{+}\nu$ events.  $\mu\,\mathrm{DIF}$ events, although the probability of occurrence is  small ($6 \times 10^{-6}$), would represent a significant background comparable to the low energy tail fraction since it has the same time distribution as \pie~ events. Thanks to the high granularity of the ATAR, it is possible to observe the energy deposition at the pion decay origin   and  to measure the local  energy loss along the positron track. Typically, a \tmu\ muon travels  0.8\,mm in the ATAR and leaves high dE/dx hits in 4 strips on average. An initial simulation of $\mu\,\mathrm{DIF}$ events, indicated a suppression factor of 20 from local dE/dx measurements and we expect another order of magnitude suppression from positron tracking, pulse detection, and total energy measurements. This would  put the $\mu\,\mathrm{DIF}$ at about $10\%$ of the tail fraction $f$. (We are also studying the possibility of reducing the LGAD strip thicknesses in the stopping region to enhance rejection of this background and/or using a separate thin layer ATAR setup for studying this effect.) Furthermore, we expect that experimental studies of observable  $\mu\,\mathrm{DIF}$ will enable us to know the background component accurately so it can be subtracted.

As illustrated in Fig.~\ref{fig:EventTypes}, another potentially significant  low energy background in the tail region comes from $\pi\,\mathrm{DIF}$ in the ATAR followed by muon  decay at rest. This component dominated the background suppressed spectrum in PIENU.
%ATAR event displays of some $\pi^{+}\rightarrow e^{+}\nu$ and $\pi^{+} \rightarrow \mu^{+} \rightarrow  e^{+}$ examples are included in the Appendix \todo{are they?}. 
Simulations indicate that 0.1\% of pions decay in flight in the ATAR before stopping and initial studies indicate that the $\pi\,\mathrm{DIF}$ events can be suppressed by a factor of 5000 using ATAR tracking information which recognizes kinks in the topology and measures dE/dx along the track. 
Along with suppression of muon decays by selecting a narrow  time window e.g.  3--35\,ns after the pion stop, we estimate that the \pdif\ contribution to the uncertainty in the tail correction $f$ will be negligible.  




==> Theory/Exotics.tex <==
%\subsection{Heavy Neutrinos and other Dark Sector Physics}
%\label{sec:BSM}

%The PIONEER experiment will also achieve improved sensitivity in probing for effects of heavy neutrinos. If a heavy neutrino has a sufficiently low
%mass that it can be emitted, the signature will be a monochromatic peak
%in the energy of the outgoing charged lepton at an anomalously low value.
%Even if the heavy neutrino has a mass greater than the kinematic limit
%for emission, there will, in general, still be an apparent violation of
%$e$--$\mu$ universality, i.e., a deviation in the measured ratio $R_{e/\mu} \equiv BR(\pi^+ \to e^+ \nu_e)/BR(\pi^+ \to \mu^+ \nu_\mu)$ from its SM value 
%\cite{Shrock:1980vy,Shrock:1980ct,Shrock:1981wq}. %Constraints from early experiments on $\pi^+_{\ell 2}$ decays were reported in 
%Refs.~\cite{Abela:1981nf,Minehart:1981fv,Bryman:1983cja,Azuelos:1986eg,Britton:1992pg}.
%Recent results on $\pi^+_{\ell 2}$ decays include
%\cite{PiENu:2015seu,PIENU:2017wbj,PIENU:2019usb}.
%Constraints from the non-observation of neutrinoless double beta
%decays imply that the heavy neutrinos of relevance here are Dirac fermions.  This
%can be arranged in various BSM scenarios.  There are also constraints
%from primordial nucleosynthesis.  Heavy neutrinos with masses of 
%relevance here are consistent with these primordial nucleosynthesis 
%constraints in several BSM theories %\cite{Arguelles:2021dqn}.
%Recent limits include \cite{Bryman:2019ssi,Bryman:2019bjg}.
%The PIONEER experiment could also search for other BSM pion decays,
%including $\pi^+ \to \ell^+ \nu_\ell X$, where $X$ is a neutral weakly
%interacting boson (a limit from PIENU is \cite{PIENU:2021clt}). 

%Looking beyond sterile neutrinos, dark sectors that consist of particles that interact very feebly with the SM are highly motivated extensions of the SM. There is an ever-growing interest in exploring the parameter space of such scenarios.  
%The PIONEER experiment will improve sensitivity to probes of effects of heavy neutrinos and will have unique capabilities to search for pion decays to various light BSM states.
% One example is the three-body decay $\pi^+ \to \ell^+ \nu_\ell X$, where $X$ could, for example, be an axion-like-particle (ALP) that mixes with the neutral pion~\cite{Altmannshofer:2019yji}, or a light gauge boson coupling to differences of lepton numbers~\cite{Dror:2020fbh}. Another interesting process is the three-body decay $\pi^+ \to \ell^+ X Y$, where both $X$ and $Y$ are light dark sector particles~\cite{Batell:2017cmf}. Existing limits from PIENU~\cite{PIENU:2021clt} already probe some of these models. Moreover, PIONEER can also look for lepton-flavor-violating decays of the muon into light BSM particles $\mu \to e X$.

==> TrainingEDI.tex <==
During the development and operation of \nexp~   particular attention will be given to maintain diversity including women and other under-represented groups as well as  in  the level of experience of the participants.  Mentorship is also an important part of the training of highly qualified personnel (HQP). Both mentors and mentees benefit from a larger group of HPQs and PIs with/from whom they can  interact, learn, and teach. Thus, it is important to have a well-balanced team of HQP and principals (PI). 


The diversity of experience is also reflected in the current PI team including very experienced PIs and early to mid-career researchers.
All PIs have significant experience in training HQP and several members have followed  training courses related to Equity, Diversity and Inclusion (EDI) aspects of supervision and have been  active in outreach in view of improving gender-balance in science. The recruitment and inclusion of women and under‐representative minorities in the PIONEER  group is a priority and the participant groups have good records. 
%\footnote{For example, 45\% of the graduate students and postdoctoral researchers hired by the rare decay group at TRIUMF/UBC since 2000 were either women or under‐represented minorities and  two female TRIUMF faculty members recently joined the group.}

We commit to providing equitable mentorship with the intention of advancing the research objectives of the group and the personal objectives of the participants. Opportunities to participate in diversity, inclusion, and equity activities as well as soft-skill and cross-sectoral training will be encouraged.

Students and PDFs will be given opportunities to present their work at conferences and collaboration meetings. Since the pandemic started many conferences turned to an online or hybrid format. While in-person meetings remain important for networking and informal idea exchanges, maintaining the pre-covid level of travel for conferences should be carefully assessed in light of environmental impact and equal opportunities for HQP. A report from  ECFA (European Committee for Future Accelerators) early career scientist panel meant as input to the 2020 European Strategy Update for particle physics (https://arxiv.org/abs/2002.02837) raised concerns about the carbon-footprint of conference-related travels and the discriminatory effect that in-person only meetings have on scientists with children (having unfortunately still a more important impact on female scientists). Thus, as far as possible, we will leave the option to the HQP to decide on an in-person or remote attendance to meetings and conferences.

The HQP in the groups will be part of an international collaboration of currently 25 research institutes and universities across USA, Europe, Canada, Japan, China and Mexico, offering many opportunities for networking in a diverse environment.
 
As far as research training is concerned, PIONEER, being a medium scale precision physics experiment, offers excellent opportunities for advanced hands-on training on a wide variety of hardware and software technologies (LXe calorimetry, cryogenic engineering, photo detectors, advanced Si detectors, state-of-the-art data acquisition, high speed electronics). Those will be complemented with training in sophisticated data analysis and simulation methods applicable to many forefront areas of experimental science but also to  industry where those skills are highly sought. 

Students and early researchers will be provided the opportunity to learn about all aspects of  the experiment leading to well rounded training for future careers in particle physics and other technical pursuits.
Students and postdoctoral researchers will take on significant and diverse individual responsibilities making them able to move to other leading high energy physics projects like the LHC, to low energy nuclear physics projects, or to industry. The experienced members of the team will mentor and instruct the more junior members in a collegial atmosphere which encourages learning and accomplishment.
Within this project, the PDF and  students will experience both the large infrastructure laboratories  and the university lab environments . They will also  work on R\&D developments and on simulations providing them with hardware and computational projects. Students will participate in the design of test assemblies, installation and data-taking  as well as data-analysis.
Some will be focusing on  simulation studies and machine-learning analyses.  


In summary HQPs on this project will benefit from an inclusive environment and the supervision of a strong group of PIs with a wide range of expertise incorporated within a larger group of experts. 

